Convex-Concave Zero-sum Markov Stackelberg Games

Zero-sum Markov Stackelberg games can be used to model myriad problems, in domains ranging from economics to human robot interaction. In this paper, we develop policy gradient methods that solve these games in continuous state and action settings using noisy gradient estimates computed from observed trajectories of play. When the games are convex-concave, we prove that our algorithms converge to Stackelberg equilibrium in polynomial time. We also show that reach-avoid problems are naturally modeled as convex-concave zero-sum Markov Stackelberg games, and that Stackelberg equilibrium policies are more effective than their Nash counterparts in these problems.

==> conc.tex <==

\amy{add to the conclusion that our work makes it possible to model reach-avoid problems as Stackelberg games. people may have had this inclination before, without the algos. we are providing such people w/ the requisite machinery.}


\amy{is invex-incave tractable?}

Perhaps more importantly, even in discrete action stochastic (Stackelberg) games, without further assumptions, it is well-established that this objective is in general not convex-concave but rather invex-incave.\deni{Add citations}

==> conclusion.tex <==
\section{Conclusion}

In this paper, we developed policy gradient methods that solve 
%\samy{zero-sum stochastic Stackelberg games}
{stochastic min-max optimization problems with coupled constraints} using noisy gradient estimates computed from observed trajectories of play.
We also introduced the class of convex-concave zero-sum stochastic Stackelberg games, and proved that our algorithms converge to a recursive (or Markov perfect) Stackelberg equilibrium in polynomial time for such games.
We then proved that reach-avoid problems are naturally modeled as convex-concave zero-sum stochastic Stackelberg games, and thus obtained polynomial-time convergence guarantees for these games as well.
%, for which our algorithm provides polynomial-time computational guarantees. 
Finally, through experiments, we showed that modeling reach-avoid problems as Stackelberg games leads to safer and livelier solutions, that are less likely to result in collisions and more likely to reach their goals, than their Nash counterparts.


==> convex-incave.tex <==
\if 0
In a reach-avoid game, a player called the attacker aims to reach a target set in the state space while steering clear of a subset of the states called unsafe states and avoiding getting intercepted by an opponent called the attacker. Reach-avoid games have applications to a large number of problems from network consensus problems in adversarial settings \cite{khanafer2013robust}, motion planning \cite{chen2014multiplayer, karaman2011sampling}, pursuit evasion games \cite{flynn1974lion, lewin1986lion}, autonomous driving \cite{leung2022learning}, and path planning to name a few \cite{zhou2018efficient}.
\fi

% Reach-avoid games are traditionally formulated as continuous-time, i.e., differential, games.
% As these games are ultimately solved via discretization, we introduce a discrete-time variant of the problem as a discounted infinite-horizon zero-sum Stackelberg game, whose solutions are Stackelberg equilibria.
% We show that the follower's action correspondence is naturally concave, which together with standard assumptions on the game satisfied by reach avoid problems, guarantees that the zero-sum stochastic Stackelberg game we propose is convex-concave, facilitating efficient solutions. 
% In experiments, our formulation improves the safety of the agent/attacker without sacrificing liveness.

% % For simplicity, we present our model for two-dimensional state, spaces but we note that our model generalizes to state space in arbitrary dimensions.
% % An infinite horizon discrete-time discounted reach avoid problem $(\states[\mathrm{free}], \states[\mathrm{obs}])$ consists of two players, the defender (or $\outeraction$-player) and the attacker (or $\inneraction$-player) who respectively occupy any location $\state[][\outeraction], \state[][\inneraction]$ in a continuous space environment $\states[\mathrm{obs}] \cup \states[\mathrm{free}] \in \R^s$ and defined by two partitions, the unobstructed space $\states[\mathrm{free}]$ through which both players can roam freely and the obstructed space $\states[\mathrm{obs}]$ which corresponds to the obstructed part of the space that no player can reach. The goal of the attacker is to reach a state $\state[][\inneraction] \in \targetstates$ in the target set $\targetstates \subset \states[\mathrm{free}]$, while steering clear from a set of joint states in the valid (or safe) set $\safestates \subset \states$. For any $r \in \R_+$, a typical choice for the safe set is  $\safestates = \{\state \in \states \mid  \|\state[][\outeraction] - \state[][\inneraction] \|^2 \leq r \}$, in which case the safe set is describing the safety radius the attacker should keep from the defender. The environment is initialized at some state $\state[0] \sim \initstates \in \simplex(\states[\mathrm{free}])$ and at any subsequent time-step $\iter \in \N_+$, the players encounter a new state $\state[\iter]$. At each time-step $\iter \in \N_+$, the defender and the attacker respectively choose a direction towards which they will head, $\outeraction[][][][\iter] \in \angles$ and $\inneraction[][][][\iter] \in \angles$, from a set of directions $\angles$. Once they have taken their actions, the players then end up in a new state determined by the players' displacement functions $\detertrans[\outeraction]: \states[\mathrm{free}] \times \angles \to \states[\mathrm{free}]$ and $\detertrans[\inneraction]: \states[\mathrm{obs}] \cup \states[\mathrm{free}] \times \angles \to \states[\mathrm{obs}] \cup \states[\mathrm{free}]$ such that $\state[\iter + 1] \doteq \left(\detertrans[\outeraction]( \state[\iter][\outeraction][\outer], \outeraction[][][][\iter]), \detertrans[\inneraction](\state[\iter][\inneraction], \inneraction[][][][\iter]) \right)$.  For convenience, we define $\detertrans[\inneraction](\state[][], \outeraction, \inneraction[][][][]) \doteq \left(\detertrans[\outeraction]( \state[][\outeraction], \outeraction[][][][]), \detertrans[\inneraction](\state[][\inneraction], \inneraction[][][][]) \right)$ A solution to the reach avoid problem is a sequence of directions $(\outeraction[][][][\iter], \inneraction[][][][\iter])_{\iter \in \iters} \in \angles^2$ s.t. for all $\iter \in \iters$, $\detertrans\left(\detertrans[\outeraction]( \state[\iter][\outeraction], \outeraction[][][][\iter]), \detertrans[\inneraction](\state[\iter][\outeraction], \inneraction[][][][\iter]) \right) \in \safestates$ and $\detertrans[\inneraction](\state[\numiters][\inneraction], \innerangle[\numiters]) \in \targetstates$. In reach-avoid problems, we are interested in solutions for which the attacker reaches the target state the quickest, however as the optimal path to take for the attacker depends on the defender's decision, we have to impose additional assumptions on the defender. 
% \arjun{copied this to the body. REMEMBER TO DELETE}
% A \mydef{(discounted infinite-horizon discrete-time and action) reach-avoid game} $(\states, \targetstates, \safestates, \initstates, \reward, \detertrans)$ comprises two players, the \mydef{defender} (or $\outeraction$-player) and the \mydef{attacker} (or $\inneraction$-player), each of whom occupies a state $\state[][\outeraction], \state[][\inneraction] \in \states$ in a continuous, compact, and convex space $\states \in \R^s$.
% % and defined by two partitions, the unobstructed space $\states[\mathrm{free}]$ through which both players can roam freely and the obstructed space $\states[\mathrm{obs}]$ which corresponds to the obstructed part of the space that no player can reach. 
% The attacker's goal is to reach a state in the target set $\targetstates \subset \states$, while steering clear of any joint
% %joint states $\state \doteq (\state[][\outeraction], \state[][\inneraction]) \in \safestates$ in the 
% invalid states $\safestates \subset \states^2$.
% (This avoid set formulation is intended to represent capture constraints, which have been the focus of the reach-avoid literature \cite{zhou2018efficient}.)
% Initially, the players occupy some state $\state[0] \sim \initstates \in \simplex(\states^2)$.
% %, and then at any subsequent time-step $\iter \in \N_+$, they encounter a new state $\state[\iter]$. 
% At each subsequent time-step $\iter \in \N_+$, the defender and the attacker respectively choose a directions in which to move, $\outeraction[][][][\iter] \in \angles$ and $\inneraction[][][][\iter] \in \angles$, from a discrete set of directions $\angles$, i.e., angles describing a direction in every dimension of the state space.
% After taking their actions, they move to a new state, as determined by their respective displacement functions which rotates and moves the players through the state space $\detertrans[\outeraction], \detertrans[\inneraction]: \states \times \angles \to \states$, i.e., $\state[\iter + 1] \doteq \left(\detertrans[\outeraction]( \state[\iter][\outeraction], \outeraction[][][][\iter]), \detertrans[\inneraction](\state[\iter][\inneraction], \inneraction[][][][\iter]) \right)$.  
% %For convenience, we define $\detertrans (\state[][], \outeraction, \inneraction[][][][]) \doteq \left(\detertrans[\outeraction] (\state[][\outeraction], \outeraction[][][][]), \detertrans[\inneraction] (\state[][\inneraction], \inneraction[][][][]) \right)$.
%  We define the payoffs of the game as
% \begin{align}
%     \reward(\state, \outeraction, \inneraction)  = - \min_{{\state[][\inneraction]}^\prime \in \targetstates}\left\| {\state[][\inneraction]}^\prime - \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \right\|^2 \enspace. \label{eq:reward_reach_avoid}
% \end{align}
%     % - \min_{}\left\|\detertrans[\inneraction](\state,  \inneraction) \right\| \in \targetstates
%     % \left\{
%     % \begin{array}{cc}
%     %     1 & \text{if $ \in \targetstates$} \\
%     %     0 & \text{otherwise}
%     % \end{array}
%     % \right.
% %\end{align}
% A solution to a reach-avoid game is a sequence of directions $(\outeraction[][][][\iter], \inneraction[][][][\iter])_{\iter \in \iters}$ 
% %$\in \angles^2$ 
% of length $\numiters$ s.t.\ for all $\iter \in \iters$, $\left( \detertrans[\outeraction]( \state[\iter][\outeraction], \outeraction[][][][\iter]), \detertrans[\inneraction] (\state[\iter][\outeraction], \inneraction[][][][\iter]) \right) \in \safestates$ and $\detertrans[\inneraction] (\state[\numiters][\inneraction], \innerangle[\numiters]) \in \targetstates$, i.e., the players never enter the avoid set and the attacker reaches the target set. 

% % \footnote{Although we assume that players randomize their choice of direction, at a Stackelberg equilibrium the attacker's equilibrium policy is always a deterministic policy as it is the solution to an MDP given the defender's policy, however, this provides the defender with more advantage and as such leads to more robust follower policies.} 
% \if 0
% In reach-avoid problems, we are interested in solutions for which the attacker reaches the target state the quickest without going through the invalid states, however as the optimal path to take for the attacker depends on the defender's decision, we have to assumptional choices on the defender. 
% % We define the space  as the space of all possible positions of the players in the unobstructed environment s.t. for any state $\state \doteq (\state[][\outeraction], \state[][\inneraction])$, $(\state[][\outeraction], \state[][\inneraction])$ denote respectively the positions of the defender and attacker.
% As such, we will assume that the attacker is adversarial and model the reach avoid problem as a zero-sum stochastic Stackelberg game between the defender who is the leader and the defender who is the follower. The state space
% % \footnote{The results and the game we present hold for $\states \doteq  (\states[\mathrm{free}] \cap \states[\mathrm{obs}])^2$ for simplicity states we model the state space as the space of unobstructed states, however}
% and initial state distribution of this zero-sum stochastic Stackelberg game is respectively given as $\states^2$ and $\initstates$, the action spaces for both players are defined as $\outeractions = \inneractions \doteq \simplex(\angles)$, while the transition probability function is deterministic and given by the displacement function $\detertrans$. We define the rewards of the game as:
% \begin{align}
%     \reward(\state, \outeraction, \inneraction)  = - \min_{\state^\prime \in \targetstates}\left\| \state^\prime - \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \right\|^2 
%     % - \min_{}\left\|\detertrans[\inneraction](\state,  \inneraction) \right\| \in \targetstates
%     % \left\{
%     % \begin{array}{cc}
%     %     1 & \text{if $ \in \targetstates$} \\
%     %     0 & \text{otherwise}
%     % \end{array}
%     % \right.
% \end{align}
% \fi

% % \deni{Need to say that since the state of the leader and follower are separate we can relax to convexity in $\state[\outer]$ and concavity in $\state[\inner]$}.

% The most important feature of this Stackelberg game is the action correspondence, defined for all states $\state \in \states$ as $\coupledactions(\state, \outeraction) \doteq \{\inneraction \in \inneractions \mid \detertrans(\state, \outeraction, \inneraction) \notin \safestates \}$. 
% %We focus on invalid state sets that represent capture constraints and which have been the focus of the reach-avoid literature \cite{zhou2018efficient}.
% A typical choice for the avoid set is the \mydef{safety radius set} $\safestates = \{\state \in \states^2 \mid \|\state[][\outeraction] - \state[][\inneraction] \|^2 \leq \varepsilon \}$, for some $\varepsilon \in \R_+$, which establishes a safe distance for the attacker to keep from the defender.
% In zero-sum stochastic Stackelberg games, capture constraints can be formulated by action correspondences of the form $\coupledactions(\state, \outeraction) \doteq \{\inneraction \in \inneractions \mid  \detertrans[\outeraction](\state[][\outeraction], \inneraction) \in \overline{\calP} + \{\detertrans[\outeraction](\state[][\outeraction], \outeraction)\} \}$, where $P \subset \R^s$ and the sum set is a capture set centered around the defender.
% %which describes how close the attacker and defender have to be for the attacker to be captured, and 
% As such, the attacker should always chose an action $\inneraction$ that takes it to a state in the complement of $\calP +  \{\detertrans[\outeraction](\state, \outeraction)\}$, i.e., $\overline{\calP} +  \{\detertrans[\outeraction](\state, \outeraction)\}$. 
% For instance, if we take $P$ to be the $c$-ball around the position at which the defender is located after taking its action, \amy{reviewer says: missing dot} i.e., $\widebar{\ball[c][{\detertrans[\outeraction](\state, \outeraction)}]}  = \widebar{\ball[c][\zeros]} +  \{\detertrans[\outeraction](\state, \outeraction)\}$ for some $c >0$, then we obtain the action correspondence:
% \begin{align}
%     \coupledactions(\state, \outeraction) \doteq \widebar{\ball[\varepsilon][\zeros]} +  \{\detertrans[\outeraction](\state, \outeraction)\}\label{eq:safety_radius_constr}
% \end{align}
% which is associated with the safety radius set. 
% Interestingly, for any choice of capture set $P$, possibly even non-convex, and any displacement function $\detertrans$ that is affine in $(\action, \otheraction)$, $\coupledactions(\state, \outeraction)$ is guaranteed to be continuous and concave in $\outeraction$ for all $\state \in \states$ (see Example 2.6 of \citeauthor{nikodem1989concave} \cite{nikodem1989concave}) Since $\angles$ is a discrete set, here affineness is defined with respect to the convex hull of $\angles$, i.e., the continuous space of angles $\simplex(\angles)$ since $\angles$ is a set of angles. We note that since the displacement function $\detertrans$ is simply describing a rotation and translation, it is an affine transformation over the space of continuous angles $\simplex(\angles)$, the example in \Cref{sec_app:experiments} illustrates this clearly in a two-dimensional setting.

% We will suppose that the players employ stochastic policies $\policy[\outeraction], \policy[\inneraction]: \states \to \simplex(\angles)$. We note that although we assume that players randomize their choice of direction, at a Stackelberg equilibrium the attacker's equilibrium policy is always a deterministic policy as it is the solution to an MDP given the defender's policy, however, this provides the defender with more advantage and as such leads to more robust follower policies. Additionally, since $\angles$ is a set of angles, randomization can be simply interpretted as picking an angle in the convex hull of discrete angles $\simplex(\angles)$.
% The following theorem shows that if we assume a bilinear parameterization, i.e., $\policy[\outeraction] \doteq \policy[\outer], \policy[\inneraction] \doteq \policy[\inner]$ for parameters $\outer \in \outerset \subset \R^\outerdim$ and $\inner \in \innerset \subset \R^\innerdim$ s.t. $(\policy[\outer](\state), \policy[\inner](\state))$ is linear in $\state$ and linear in $(\outer, \inner)$, we guarantee the assumptions of \Cref{lemma:convexity_params_leader} and \Cref{lemma:concavity_params_follower}, and can compute a solution to this game in polynomial-time via nested policy gradient descent ascent (\Cref{alg:nested_pgda}). 
% % \deni{Add that affine-ness is very natural for transition probability function, since in two and three dimensional reach avoid the transition is a rotation, which IS an affine transform, so this solves already studied dubbins car problems not only in 2d but also 3d.}

% At each time-step $\iter \in \N_+$, the defender and the attacker respectively choose a direction towards which they will head, $\outeraction[][][][\iter] \in \angles$ and $\innerangle \in \angles$, from a set of directions $\angles \doteq \{-1, 0, 1\}$, s.t. $-1$ corresponds to a left turn, $0$ corresponds to keeping straight, and $1$ corresponds to a right turn.

% The defender and the attacker are both characterized by some respective velocities $\outervel \in \R^{\numstates}$ and $\innervel \in \R^{\numstates}$ that characterizes the change in the player's rate of change in the players' position in the state space\footnote{More generally, our results apply when the velocities are state-dependent, bur for ease of presentation we assume that they are constant.}


==> deterministic_policy_critic.tex <==

\subsection{Nested Deterministic Policy Actor Critic}
More precisely, recall that the seminal \mydef{(deterministic) policy gradient theorem} \cite{sutton1999policy, silver2014deterministic} provides sufficient assumptions (\Cref{assum:smooth}) for the state-value function of any Markov decision process (MDP) \cite{bellman1952theory}, and hence the cumulative utility function of an MDP to be differentiable with respect to the parameters of a Lipschitz-continuous policy parameterization. A straightforward generalization of this result holds under \Cref{assum:smooth} for differentiating the cumulative utility $\cumulutil$ associated with any zero-sum stochastic Stackelberg game w.r.t the parameters $\outer$ and $\inner$ of any Lipschitz-continuous parameterization at any point $(\outerpoint, \innerpoint) \in \outerset \times \innerset$
% and $\inner$
% . In particular, under \Cref{assum:zero_exist}, we have:
\begin{align}
    % &\grad[\outer] \cumulutil(\outer, \inner) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\initstates][{(\outer, \inner)}]\\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}}  \left[ \actionvalue[][{(\outer, \inner)}](\staterv, \actionrv)  \log \left(\grad[\outer] \policy[\outer](\actionrv \mid \staterv)\right) \right] 
    % &\grad[\inner] \cumulutil(\outer, \inner) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\initstates][{(\outer, \inner)}]\\ \actionrv \sim \policy[\inner](\cdot \mid \staterv)}}  \left[ \actionvalue[][{(\outer, \inner)}](\staterv, \actionrv)  \log \left(\grad[\inner] \policy[\inner](\actionrv \mid \staterv)\right) \right] \\
    &\grad[\outer] \cumulutil(\outerpoint, \innerpoint) = \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    }  \left[\grad[\outeraction] \actionvalue[][{(\outerpoint, \innerpoint)}](\staterv, \policy[\outerpoint](\staterv), \policy[\innerpoint](\staterv))  \grad[\outer] \policy[\outerpoint](\staterv) \right] 
    &\grad[\inner] \cumulutil(\outerpoint, \innerpoint) = \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    }  \left[\grad[\inneraction] \actionvalue[][{(\outerpoint, \innerpoint)}](\staterv, \policy[\outerpoint](\staterv), \policy[\innerpoint](\staterv))  \grad[\inner] \policy[\outerpoint](\staterv) \right]\\ 
    % \\
\end{align}

However, in order for nested stochastic gradient descent ascent to run efficiently, we need to compute an unbiased estimate of the gradient of the game Lagrangian $\lang(\inner, \langmult; \outer)$ from trajectory samples $\{\hist[\numsample]\}_{\numsample = 1}^\numsamples \sim \histdistrib$ since we do not have access to the state visitation distribution $\histdistrib$. Using the deterministic policy gradient theorem, we can deduce that the gradient of the game Lagrangian with respect to $\outer$ and $\inner$ are respectively given as:
\begin{align}
    \grad[\outer] \lang(\inner, \langmult; \outer) \doteq \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    }  \left[\grad[\inneraction] \actionvalue[][{(\outerpoint, \innerpoint)}](\staterv, \policy[\outerpoint](\staterv), \policy[\innerpoint](\staterv))  \grad[\inner] \policy[\outerpoint](\staterv) \right]  + \left< \policy[\langmult], \grad[\outer] \constr[](\policy[\outer], \policy[\inner]) \right>\\
    \grad[\inner] \lang(\inner, \langmult; \outer) \doteq \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    }  \left[\grad[\outeraction] \actionvalue[][{(\outerpoint, \innerpoint)}](\staterv, \policy[\outerpoint](\staterv), \policy[\innerpoint](\staterv))  \grad[\outer] \policy[\outerpoint](\staterv) \right] + \left< \policy[\langmult], \grad[\inner] \constr[](\policy[\outer], \policy[\inner]) \right>
\end{align}

\begin{assumption}[Smoothness Assumptions]
\label{assum:smooth}
Consider the zero-sum stochastic Stackelberg game $\initgame$ and a paraterized policy profile $(\policy[\outer], \policy[\inner])$.
Suppose that for all states $\state, \state^\prime \in \states$, 1.~$\trans(\state \mid \state^\prime, \outeraction, \inneraction), \reward(\state, \outeraction, \inneraction),  \constr[][1](\state, \outeraction, \inneraction), \ldots, \constr[][\numconstrs](\state, \outeraction, \inneraction), \policy[\outer](\state), \policy[\inner](\state)$ are Lipschitz-continuous in $(\outer, \inner)$, 
and
2.~(Slater's condition) 
$\forall \outeraction \in \outeractions, \exists \widehat{\inneraction} \in \inneractions$ s.t.\ $\constr[][\numconstr](\state, \outeraction, \widehat{\inneraction}) > 0$.
% , and
% 3.~ $\grad[\outer] \policy[\outer]$, $\grad[\inner] \policy[\inner]$ continuous in $\outer$ and $\inner$ respectively, $\grad[(\outeraction, \inneraction)] \trans, \grad[(\outeraction, \inneraction)] \reward$ are continuous in $(\outeraction, \inneraction)$.
%\deni{N.B. Any continuously differentiable function is continuous.} 
% 4.~the marginal function $\val(\outer)$ is convex in $\outer$; and
% 5.~$\obj[\obji], \constr[\constri][1], \hdots, \constr[\constri][\numconstrs]$ are concave in $\inner$ for all $\outer \in \outerset$.
\end{assumption}

In order to compute these gradients, we have to in turn be able to compute the gradient of the action-value function $\qfunc[][{(\outerpoint, \innerpoint)}]$. This is a challenging task since we do not have access to the reward or transition function of the game. To overcome this issue, we can estimate the true action-value function via function approximation from sample trajectories. That is, for any policy profile $(\policy[\outerpoint], \policy[\innerpoint])$, instead of using the true action-value function, we will compute a \mydef{critic function} $\qfunc[ ][\weight]: \states \times \outeractions \times \inneractions \to \R$ which is parametrized by some weights $\weight \subset \R^\omega$ such that $\qfunc[ ][\weight](\state, \outeraction, \inneraction) \approx \qfunc[ ][{(\outerpoint, \innerpoint)}](\state, \outeraction, \inneraction)$. Unfortuntely, in general substituting the true value function with the critic function might induce bias and as a result nested stochastic gradient descent will not necessarily follow the
true gradient of the game Lagrangian. 

To overcome the issue of bias, \citeauthor{silver2014deterministic} \cite{silver2014deterministic} introduce the class of \mydef{compatible critic function}, i.e., critic networks $\qfunc[ ][\weight]$ such that 1.~ $\grad[(\outeraction, \inneraction)] \qfunc[ ][\weight] = \weight^T \left[ \grad[(\outer, \inner)](\policy[{\outer[][][][]}](\state), \policy[{\inner[][][][]}](\state))\right]$, and 2.~ $\Ex_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]} \left[ \left\|\grad[(\outer, \inner)]\qfunc[ ][\weight](\staterv, \policy[\outerpoint](\staterv), \policy[\innerpoint](\staterv)) - \grad[(\outer, \inner)]\qfunc[ ][{\outerpoint, \innerpoint}](\staterv, \policy[\outerpoint](\staterv), \policy[\innerpoint](\staterv)) \right\|^2_2\right]$ is minimized. We note that there always exists an affine compatible critic function of the form: $\qfunc[ ][\weight](\state, \outeraction, \inneraction; \outer[][][], \inner[][][]) \doteq \weight^T \left[ \grad[(\outer, \inner)](\policy[{\outer[][][][]}](\state), \policy[{\inner[][][][]}](\state))\right] \left[(\outeraction, \inneraction) - (\policy[{\outer[][][][]}](\state), \policy[{\inner[][][][]}](\state)) \right] + \vfunc[ ][\weight](\state)$ where $\vfunc[ ][\weight]: \states \to \R$ is an affine function of $\weight$ and any feature function of $\state$. The affine structure of this compatible critic function in $\weight$ implies that a compatible critic function can be computed efficiently under suitable assumptions with even a closed form solution.  Hereforth, we will restrict ourselves only to compatible critic functions $\qfunc[][\weight]$.

% \begin{assumption}[Parametrization Assumption]\label{assum:affine_param}
% Consider the policies $\policy[\outer]$, $\policy[\inner]$, and the KKT system $\policy[\langmult]$. 1.~ $\policy[\outer]$, $\policy[\inner]$, and $\policy[\langmult]$ are respectively continuous and affine in $\outer$, $\inner$, and $\langmult$. 
% \end{assumption}
% Using the policy gradient theorem, an application of Danskin's theorem \cite{danskin1966thm} can allow us obtain the gradient of the marginal function $\marginalfunc$ at any point $\outer$ at which it is differentiable:
% \begin{align}
%     \grad[\outer] \marginalfunc(\outer) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\initstates][{(\outer, \inner[][][*](\outer))}]\\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}}  \left[ \actionvalue[][{(\outer, \inner[][][*](\outer))}](\staterv, \actionrv)  \log \left(\grad[\outer] \policy[\outer](\actionrv \mid \staterv)\right) \right]
% \end{align}
% \noindent where $\inner[][][*](\outer) \in \argmax_{\inner \in \innerset} \cumulutil(\outer, \inner)$ is the best-response policy with parameters $\outer$.




 With the stochastic game Lagrangian defined, we 

\begin{algorithm}[H]
% \caption{Nested Stochastic Gradient Descent Ascent / Max-Oracle Stochastic Gradient Descent}
\textbf{Inputs:} $\outerset, \innerset, \util, \outer[][][][0], \inner[][][][0], \langmult[][][0], \numiters[\outer], \numiters[\inner], \left\{\learnrate[\outer][\iter] \right\}_{\iter = 0}^{\numiters[\outer]-1}, \left\{\learnrate[\inner][\iter] \right\}_{\iter = 0}^{\numiters[\outer]-1}$\\
\textbf{Outputs:} $(\outer[][][][\iter], \inner[][][][\iter])_{\iter = 0}^{\numiters[\outer]-1}$
\begin{algorithmic}[1]\label{alg:nested_pgda}
\caption{Nested Deterministic Policy Actor Critic}
\State $\inner[][][][] \gets  \inner[][][][0]$
\State $\langmult[][][] \gets  \langmult[][][0]$
\For{$\iter = 0, \hdots, \numiters[\outer] - 1$}
        \For{$s = 0, \hdots, \numiters[\inner] - 1$}
            \State Sample trajectories $\{\hist[\numsample][][]\}_{\numsample = 1}^\numsamples  \sim \histdistrib[][{(\outer[][][][\iter], \inner[][][][\iter])}]$ and observe rewards $\{\rewards[\numsample]\}_{\numsample = 1}^\numsamples = \{(\rewards[\numsample][\numhorizon])_{\numhorizon}\}_{\numsample}$
            \State Find $\weight \in \R^\omega$ s.t. $\min_{\weight \in \R^\omega} \sum_{\numsample}\left\| \rewards[\numsample][\iter] - \qfunc[ ][\weight](\state, \outeraction, \inneraction; \outer[][][][\iter], \inner[][][][\iter])]\right\|^2_2$
            \State $\inner[][][] \gets  \project[\innerset] \left[\inner[][][] + \nicefrac{1}{\numsamples}\sum_{\numsample}\grad[\inner] \lang[{\hist[\numsample]}](\inner[][][], \langmult[][]; \outer[][][][\iter]) \right]$
            \State  $\langmult[][][] \gets  \project[\langmults]\left[\langmult[][][] - \nicefrac{1}{\numsamples} \grad[\langmult] \lang[{\hist[\numsample]}](\inner[][][][], \langmult[][][]; \outer[][][][\iter]) \right]$
        % \State \textbf{IISE:}
        % \IndState[0] $\inner[][][] \gets  \project[\{\innerset: \constr(\outer, \inner) \geq \zeros \}]\left[\inner[][][] + \grad[\inner] \lang[\obji, \constri](\inner[][][], \langmult[][]; \outer[][][][\iter]) \right]$
        % \IndState[0] $\langmult[][][] \gets  \project[\R^\numconstrs_+]\left[\langmult[][][] - \grad[\langmult] \lang[\obji, \constri](\inner[][][][\iter], \langmult[][][\iter]; \outer[][][][\iter]) \right]$
        \EndFor
    \State $\inner[][][][\iter] \gets  \inner[][][][]$
    \State $\langmult[][][\iter] \gets  \langmult[][][]$
    \State Sample trajectories $\{\hist[\numsample][][]\}_{\numsample = 1}^\numsamples  \sim \histdistrib[][{(\outer[][][][\iter], \inner[][][][\iter])}]$ and observe rewards $\{\rewards[\numsample]\}_{\numsample = 1}^\numsamples = \{(\rewards[\numsample][\numhorizon])_{\numhorizon}\}_{\numsample}$
    \State Find $\weight \in \R^\omega$ s.t. $\min_{\weight \in \R^\omega} \sum_{\numsample}\left\| \rewards[\numsample][\iter] - \qfunc[ ][\weight](\state, \outeraction, \inneraction; \outer[][][][\iter], \inner[][][][\iter])]\right\|^2_2$
    \State $\outer[][][][\iter + 1] \gets \project[\outerset]\left[\outer[][][][\iter] + \nicefrac{1}{\numsamples} \grad[\outer] \lang[{\hist[\numsample]}](\inner[][][][\iter], \langmult[][][\iter]; \outer[][][][\iter]) \right]$
\EndFor
\State \Return $(\outer[][][][\iter], \inner[][][][\iter])_{\iter = 0}^{\numiters[\outer]-1}$ 
\end{algorithmic}\label{alg:nested_sgda}
\end{algorithm}

% \begin{algorithm}[H]\label{alg:nested_pgda}
% \caption{Nested (Policy) Gradient Descent Ascent}
% \textbf{Inputs:} $\outerset, \innerset, \util, \outer[][][][0], \inner[][][][0], \numiters[\outer], \numiters[\inner], \left\{\learnrate[\outer][\iter] \right\}_{\iter = 0}^{\numiters[\outer]-1}, \left\{\learnrate[\inner][\iter] \right\}_{\iter = 0}^{\numiters[\outer]-1}$\\
% \textbf{Outputs:} $(\outer[][][][\iter], \inner[][][][\iter])_{\iter = 0}^{\numiters[\outer]-1}$
% \label{alg:value_iter}
% \begin{algorithmic}[1]
% \State $\inner[][][][] \gets  \inner[][][][0]$
% \For{$\iter = 0, \hdots, \numiters[\outer] - 1$}
%     \For{$s = 0, \hdots, \numiters[\inner] - 1$}
%         \State $\inner[][][] \gets  \project[\innerset]\left[\inner[][][] + \grad[\inner] \cumulutil(\outer[][][][\iter], \inner[][][]) \right]$
%     \EndFor
%     \State $\inner[][][][\iter] \gets  \inner[][][][]$
%     \State $\outer[][][][\iter + 1] \gets  \project[\outerset]\left[\inner[][][] + \grad[\outer] \cumulutil(\outer[][][][\iter], \inner[][][][\iter])\right]$
% \EndFor
% \State \Return $(\outer[][][][\iter], \inner[][][][\iter])_{\iter = 0}^{\numiters[\outer]-1}$ 
% \end{algorithmic}
% \end{algorithm}

==> discrete_reach_avoid.tex <==
A (discrete-time discounted infinite-horizon discrete-action) \mydef{reach-avoid game} 
% \deni{What is $s$ supposed to be?} \amy{the dimensionality of the state space. but maybe it is $n$? what is $n$? you use it as well later, but i could not find it's definition.}
$(\numstates, \states, \targetstates, \safestates, \directions[\outeraction], \directions[\inneraction],  \initstates, \reward, \detertrans)$ comprises two players, the \mydef{defender} (or $\outeraction$-player) and the \mydef{attacker} (or $\inneraction$-player), each of whom occupies a state $\state[][\outeraction], \state[][\inneraction] \in \states$ in a state space $\states \subset \R^\numstates$, for some $\numstates \in \N$.
% and defined by two partitions, the unobstructed space $\states[\mathrm{free}]$ through which both players can roam freely and the obstructed space $\states[\mathrm{obs}]$ which corresponds to the obstructed part of the space that no player can reach. 
The attacker's goal is to reach a state in the target set $\targetstates \subset \states$, while steering clear of the avoid set
%joint states $\state \doteq (\state[][\outeraction], \state[][\inneraction]) \in \safestates$ in the 
$\safestates \subset \states \times \states$.
This avoid set formulation is intended to represent capture constraints, which have been the focus of the reach-avoid literature \cite{zhou2018efficient}.

Initially, the players occupy some state $\state[0] \sim \initstates \in \simplex \left( \states^2 \setminus (\safestates \cup \targetstates) \right)$ drawn from an initial joint distribution $\initstates$ over all states, excluding the target and avoid sets.
%, and then at any subsequent time-step $\iter \in \N_+$, they encounter a new state $\state[\iter]$. 
At each subsequent time-step $\iter \in \N_+$, the defender (resp.\@ attacker) chooses a distribution $\outeraction[][][][\iter] \in \outeractions \doteq \simplex(\directions[\outeraction])$ (resp.\@ $\inneraction[][][][\iter] \in \inneractions \doteq \simplex(\directions[\inneraction])$) over a discrete set of directions $\directions[\outeraction]$ (resp.\@ $\directions[\inneraction]$) in which to move \samy{}{one step} \amy{some sort of fixed amount, n'est-ce pas?}.
% , e.g., for $\numstates = 2$, these directions can be vectors $(-1,0)$ and $(1,0)$ denoting respectively the defender's (resp. attacker's) displacement one unit to the left and right
% \footnote{Note that, any set of angles in $n > 1$ dimensions can be described as a polytope $[0, 2\pi]^{n-1}$. Importantly, this set can be expressed  as a set of probability distribution over the set $[0, 2\pi]^{n-1} = \simplex(\{0, 2\pi\}^{n-1})$, meaning that the game can be interpretted as a discrete and continuous action game both}
Once the defender's and attacker's respective decisions $\direction[][\iter] \doteq (\direction[\outeraction][\iter], \direction[\inneraction][\iter])  \sim \outeraction[][][][\iter] \times \inneraction[][][][\iter]$ are realized, the game either ends with probability $1-\discount$, for some discount rate $\discount \in (0, 1)$, or
% with probability $\discount\outeraction[][{\direction[\outeraction]}][][\iter]\inneraction[][{\direction[\inneraction]}][][\iter]$ } 
the players move to a new state $\state[\iter + 1] \doteq \detertrans[\outeraction] ( \state[\iter], \direction) = \left(\detertrans[\outeraction] ( \state[\iter][\outeraction], \direction[\outeraction]), \detertrans[\inneraction] (\state[\iter][\inneraction], \direction[\inneraction]) \right)$, as determined by their respective displacement functions $\detertrans[\outeraction]: \states \times \directions[\outeraction] \to \states$ and $\detertrans[\inneraction]: \states \times \directions[\inneraction] \to \states$.
\samy{}{Although these displacement functions are deterministic, they induce} a probability transition function from state $\state$ to state $\state[][][\prime]$ because the players choose distributions $(\outeraction, \inneraction) \in \outeractions \times \inneractions$, namely $\trans(\state[][][\prime] \mid \state, \outeraction, \inneraction) \doteq \Pr(\detertrans(\state, \directionrv) = \state[][][\prime] \mid \directionrv \sim \outeraction \times \inneraction)$.

\samy{}{It remains to define the game's rewards.
While it is common to model constraints as negative rewards,} we instead define the feasible action correspondence as $\coupledactions(\state, \outeraction) \doteq \{ \inneraction \in \inneractions \mid \detertrans (\state, \direction[\outeraction], \direction[\inneraction]) \notin \safestates, \forall \direction[\outeraction] \in \supp (\outeraction), \direction[\inneraction] \in \supp (\inneraction) \}$, for all states $\state \in \states$ and actions $\outeraction \in \outeractions$; and, overloading notation, the feasible policy correspondence as $\coupledactions (\policy[\outeraction]) \doteq \{ \policy[\inneraction] : \states \to \inneractions \mid \policy[\inneraction] (\state) \in \coupledactions (\state, \policy[\outeraction] (\state)), \text{ for all } \state \in \states \}$. 
\samy{}{We are then free to define rewards  \amy{payoffs?} simply as} $\reward(\state, \outeraction, \inneraction)  = \setindic[{\targetstates}] (\state[\inneraction])$ s.t.\@ the attacker earns a reward of $1$ if it enters the target set, and $0$ otherwise.
\amy{do we need to specify what happens if there are no feasible actions? namely that the attacker has been captured, and earns 0 reward ever after? actually, is this what happens? or does the defender win, meaning the reward is then $-1$?}

% The cumulative expected payoff (resp. loss) of the attacker (resp. defender) is given by $\cumulutil(\policy[\outeraction], \policy[\inneraction]) \doteq \sum_{\iter = 0}^\infty \discount^\iter \reward(\state[\iter], \policy[\outeraction] (\state[\iter]), \policy[\inneraction] (\state[\iter]))$ where for all $\iter \in \N$, $\state[\iter + 1] \doteq \detertrans( \state[\iter], \policy(\state[\iter]))$.

%Analogously to definitions in \Cref{sec:policy_grad}, we also define the $\util$, $\statevalue$, $\statedist$ etc.
% is deterministic and given by $\detertrans \doteq (\detertrans[\outeraction], \detertrans[\inneraction]): \states^2 \times \outeractions \times \inneractions \to \states^2$

\amy{isn't it the case that an SE or GNE would necessarily only consider feasible solutions? so isn't this redundant?}
\samy{A \mydef{feasible solution} to a reach-avoid game is a policy profile $\policy \doteq (\policy[\outeraction], \policy[\inneraction]) \in \outeractions^\states \times \inneractions^\states$ 
% $(\outeraction[][][][\iter], \inneraction[][][][\iter])_{\iter  = 0}^\infty$ 
%$\in \angles^2$ 
s.t.\@ for all $\iter \in \N$, no state %that is encountered with positive probability 
in the support of $\statedist[{\initstates}][\policy]$ is in the avoid set, i.e., for all $\state \in \supp (\statedist[{\initstates}][\policy])$, $\state \notin \safestates$; and the attacker reaches the target set and remains there, i.e., there exists a $k \in \N$ s.t.\@ for all $\iter \geq k$ and $\hist \in \hists[\policy][\iter]$, we have $\{ \state[\tau][\inneraction]\}_{\tau = k}^\iter \subset \targetstates$.}{} \amy{how does $\state[\tau][\inneraction]$ relate to $\hist$?}

\if 0
\amy{this doesn't sound important to me. at least not right now. maybe move to later, when it becomes important.}
\amy{where is $\detertrans$ defined? we deleted: 
The dynamics of the car then evolve according to $\dot{x} = v\cos\theta, \dot{y} = v\cos\theta, \theta = \action$, for some magnitude $v \in \R_{++}$.}
\fi

%For convenience, we define $\detertrans (\state[][], \outeraction, \inneraction[][][][]) \doteq \left(\detertrans[\outeraction] (\state[][\outeraction], \outeraction[][][][]), \detertrans[\inneraction] (\state[][\inneraction], \inneraction[][][][]) \right)$.
% \sdeni{ We define the payoffs of the game as
% % \begin{align}
%     $\reward(\state, \outeraction, \inneraction)  = - \min_{{\state[][\inneraction]}^\prime \in \targetstates}\left\| {\state[][\inneraction]}^\prime - \state[][\inneraction] \right\|^2$. 
    % \label{eq:reward_reach_avoid}

A typical solution concept for reach-avoid games is \mydef{generalized Nash equilibrium} \cite{laine2023computation, margellos2011hamilton}: a policy profile $(\policy[\outeraction][][*], \policy[\inneraction][][*]) \in \outeractions^\states \times \coupledactions(\policy[\outeraction][][*])$ s.t. $\max_{\policy[\inneraction]  \in \coupledactions (\policy[\outeraction][][*])}\cumulutil(\policy[\outeraction][][*], \policy[\inneraction]) \leq \cumulutil(\policy[\outeraction][][*], \policy[\inneraction][][*]) \leq \min_{\policy[\outeraction]} \cumulutil(\policy[\outeraction], \policy[\inneraction][][*])$. 
Instead, we will focus on (recursive) Stackelberg equilibrium (see \Cref{sec:policy_grad}).
%
%Suppose the leader's policy is parameterized by $\outer \in \outerset \subset \R^{|\directions[\outeraction]| \times \numstates}$, while the follower's policy is parameterized by $\inner \in \innerset \subset \R^{|\directions[\inneraction]| \times \numstates}$ so that $(\policy[\outeraction],  \policy[\inneraction]) \doteq (\policy[\outer], \policy[\inner])$.
The next assumption guarantees that a reach-avoid game is a convex-incave zero-sum Markov Stackelberg game:

%under softmax policies, i.e., $\policy[\outer] (\state)= \mathrm{softmax} (\outer \state)$ and $\policy[\inner] (\state)= \mathrm{softmax} (\inner \state)$, where $\mathrm{softmax}(\w) \doteq \frac{\exp (\w \state)}{\int_{\states} \exp (\w \state) d\state}$.

% \amy{i am dumbfounded by this reward function! this has nothing to do with the (extensive!) conversations we had in my office. we only ever talked about rewards when the game ends. actually, when does the game end? you haven't mentioned the end of the game. i thought the rewards were something like, the attacker wins if they reach the target set, at which point the game ends immediately. and the defender wins if the game times out.}
% \amy{btw, is that what people mean when they say ``reward shaping''? introducing fake rewards to make the learning faster. if so, let's define the true rewards of the game, and then mention that learning was slow, so we introduced some other rewards to speed things up, if that is in fact what is going on here.}
% \amy{also, is this choice of distance function important b/c it is convex. if so, say so.}

% \amy{optimal solution!?! EQM!!! and ``sequence of directions?!'' policy! for readability, it is essential to use the technical language of the paper.}

% \footnote{Although we assume that players randomize their choice of direction, at a Stackelberg equilibrium the attacker's equilibrium policy is always a deterministic policy as it is the solution to an MDP given the defender's policy, however, this provides the defender with more advantage and as such leads to more robust follower policies.} 

\if 0
In reach-avoid problems, we are interested in solutions for which the attacker reaches the target state the quickest without going through the invalid states, however as the optimal path to take for the attacker depends on the defender's decision, we have to assumptional choices on the defender. 
% We define the space  as the space of all possible positions of the players in the unobstructed environment s.t. for any state $\state \doteq (\state[][\outeraction], \state[][\inneraction])$, $(\state[][\outeraction], \state[][\inneraction])$ denote respectively the positions of the defender and attacker.
As such, we will assume that the attacker is adversarial and model the reach avoid problem as a zero-sum stochastic Stackelberg game between the defender who is the leader and the defender who is the follower. The state space
% \footnote{The results and the game we present hold for $\states \doteq  (\states[\mathrm{free}] \cap \states[\mathrm{obs}])^2$ for simplicity states we model the state space as the space of unobstructed states, however}
and initial state distribution of this zero-sum stochastic Stackelberg game is respectively given as $\states^2$ and $\initstates$, the action spaces for both players are defined as $\outeractions = \inneractions \doteq \simplex(\angles)$, while the transition probability function is deterministic and given by the displacement function $\detertrans$. We define the rewards of the game as:
%
\begin{align}
    \reward(\state, \outeraction, \inneraction)  = - \min_{\state^\prime \in \targetstates}\left\| \state^\prime - \detertrans[\inneraction] (\state[][\inneraction],  \inneraction) \right\|^2 
    % - \min_{}\left\|\detertrans[\inneraction] (\state,  \inneraction) \right\| \in \targetstates
    % \left\{
    % \begin{array}{cc}
    %     1 & \text{if $ \in \targetstates$} \\
    %     0 & \text{otherwise}
    % \end{array}
    % \right.
\end{align}
\fi

% \deni{Need to say that since the state of the leader and follower are separate we can relax to convexity in $\state[\outer]$ and concavity in $\state[\inner]$}.

\begin{assumption}
\label{assum:reach_avoid}
    %\sdeni{}{Given a reach-avoid game $(\numstates, \states, \targetstates, \safestates, \directions[\outeraction], \directions[\inneraction],  \initstates, \reward, \detertrans)$},   
    1.~The target set $\targetstates$ is non-empty and compact;
    2.~the leader's policy is parameterized by $\outer \in \outerset \subset \R^{|\directions[\outeraction]| \times \numstates}$, while the follower's policy is parameterized by $\inner \in \innerset \subset \R^{|\directions[\inneraction]| \times \numstates}$;
    3.~the players' parameter spaces $\outerset$ and
    $\innerset$ are non-empty, compact, and convex; and
    4.~the players use softmax policies, i.e., $\policy[\w] (\state) = 
    %$\policy[\outer] (\state) = \mathrm{softmax}(\outer \state)$ and $\policy[\inner] (\state) = \mathrm{softmax}(\inner \state)$, where
    %$\mathrm{softmax}(\w \state) \doteq 
    \frac{\exp (\w \state)}{\int_{\states} \exp (\w \state) d\state}$.
    % 3.~ the state space $\states$ is continuous and the displacement function $\state \mapsto \detertrans(\state, \direction)$ is affine for all directions $\direction \in \directions[\outeraction] \times \directions[\inneraction]$.}
    % 3.~ for all states $\state \in \states$, the correspondence $\outeraction \mapsto \coupledactions(\state, \outeraction)$ continuous, concave and non-empty-, compact-valued.
\end{assumption}

Parts 1 is a standard assumption commonly imposed on reach-avoid games (see, for instance \citet{fisac2015reach}). 
Parts 2, 3, and 4 are popular parameterization assumptions \amy{proofread!} (see, for instance, Section 5 of \citet{agarwal2020optimality}).
Importantly, when the state space is discrete, this parameterization is complete in the sense that it can express all actions in the action spaces $\outeractions$ and $\inneractions$. 
The following theorem states that under \Cref{assum:reach_avoid}, the reach-avoid game is convex-incave, and can thus be solved in polynomial time via saddle-point-oracle gradient descent. \amy{did we prove this?}

% Part 3, combined with the previous assumptions, is sufficient to prove that the attacker's value function is (log-)concave in its parameters, however this assumption can entirely be done away with and one instead can settle for incavity (more specifically gradient dominance---see for instance section 5 of, \citet{agarwal2020optimality}) in the parameters for which \Cref{alg:nested_sgda} converges to a Stackelberg equilibrium in polynomial-time.

% \if 0 
% Part 3 is a natural assumption which is guaranteed to hold for many avoid sets of interest in practice. For instance, a typical choice for the avoid set is $\safestates \doteq \{ \state \in \states^2 \mid \|\state[][\outeraction] - \state[][\inneraction] \|^2 \ \leq \varepsilon \}$, for some $\varepsilon \in \R_+$, which establishes a safe distance for the attacker to keep from the defender. The associated feasible action correspondence can then be written as $\coupledactions(\state, \outeraction) \doteq \widebar{\ball[\varepsilon][\zeros]} + \{ \detertrans[\outeraction] (\state[][\outeraction], \direction[\outeraction]) \mid \forall \direction[\outeraction] \in \supp (\outeraction)\}- \state[\inneraction]$ and is in fact concave when .\footnote{\sdeni{}{More generally, we note that feasible action correspondences which enforce a safety area around the defender can be written in the form $\coupledactions( \state, \outeraction) \doteq \overline{\calP} + 
% % \{ \inneraction \in \inneractions \mid  \detertrans[\outeraction] (\state[][\outeraction], \inneraction) \in  +
% \{ \detertrans[\outeraction] (\state[][\outeraction], \outeraction) \mid \forall \direction[\outeraction] \in \supp (\outeraction)\} \}$, where $\calP \subset \R^\numstates$ is a capture set centered around the defender, and are guaranteed to be concave (see Example 2.5, 2.12, 2.15 \citet{nikodem1989concave}).}}
% % The most important feature \amy{the most important feature!!??} of this Stackelberg game is the action correspondence \amy{it is NOT even part of the game definition!}, defined for all states $\state \in \states$ as $\coupledactions(\state, \outeraction) \doteq \{ \inneraction \in \inneractions \mid \detertrans(\state, \outeraction, \inneraction) \notin \safestates \}$. 
% %We focus on invalid state sets that represent capture constraints and which have been the focus of the reach-avoid literature \cite{zhou2018efficient}.
% % 
% In zero-sum stochastic Stackelberg games, capture constraints can be formulated by action correspondences of the form $\coupledactions( \state, \outeraction) \doteq \{ \inneraction \in \inneractions \mid  \detertrans[\outeraction] (\state[][\inneraction], \inneraction) \in \overline{\calP} + \{ \detertrans[\outeraction] (\state[][\outeraction], \outeraction)\} \}$, where $\calP \subset \R^s$ is a capture set centered around the defender.
% %which describes how close the attacker and defender have to be for the attacker to be captured, and 
% As such, the attacker should always chose an action $\inneraction$ that takes it to a state in the complement of $\calP + \{ \detertrans[\outeraction] (\state, \outeraction)\}$, i.e., $\overline{\calP} +  \{ \detertrans[\outeraction] (\state, \outeraction) \}$. \amy{define $+$}
% For instance, if we take $\calP$ to be the $c$-ball around the position at which the defender is located after taking its action, \amy{reviewer says: missing dot} i.e., $\widebar{\ball[c][{\detertrans[\outeraction] (\state, \outeraction)}]}  = \widebar{\ball[c][\zeros]} +  \{ \detertrans[\outeraction] (\state, \outeraction)\}$ for some $c >0$, then we obtain the action correspondence:
% % \begin{align}
%     $\coupledactions(\state, \outeraction) \doteq \widebar{\ball[\varepsilon][\zeros]} +  \{ \detertrans[\outeraction] (\state, \outeraction)\}$
%     % \label{eq:safety_radius_constr}
% % \end{align}
% which is associated with the safety radius set. 
% Interestingly, for any choice of capture set $\calP$, possibly even non-convex, and any displacement function $\detertrans$ that is affine in $(\action, \otheraction)$ \amy{doesn't type check; $\detertrans$ is not a function of $(\action, \otheraction)$}, $\coupledactions(\state, \outeraction)$ is guaranteed to be continuous and concave in $\outeraction$, for all $\state \in \states$ (see Example 2.6 of \citeauthor{nikodem1989concave} \cite{nikodem1989concave}). 
% % Since $\angles$ is a discrete set, here affineness is defined with respect to the convex hull of $\angles$, i.e., the continuous space of angles $\simplex(\angles)$ since $\angles$ is a set of angles.
% % 
% A \mydef{bilinear parameterization}, i.e., $\policy[\outeraction] \doteq \policy[\outer], \policy[\inneraction] \doteq \policy[\inner]$ for parameters $\outer \in \outerset \subset \R^\outerdim$ and $\inner \in \innerset \subset \R^\innerdim$ s.t.\ $(\policy[\outer] (\state), \policy[\inner] (\state))$ is linear in $\state$ and linear in $(\outer, \inner)$.\amy{i don't get it, but writing is probably fine?}
% % \deni{Add that affine-ness is very natural for transition probability function, since in two and three dimensional reach avoid the transition is a rotation, which IS an affine transform, so this solves already studied dubbins car problems not only in 2d but also 3d.}
% \amy{EDIT:} \arjun{We formalize this as \Cref{thm:reach-avoid}}\sarjun{(see \Cref{sec:reach-avoid})}{with the proof in \Cref{proof:reach-avoid}}.
% \fi 

\begin{restatable}{theorem}{thmreachavoid}
\label{thm:reach_avoid}
    Any reach-avoid game $(\numstates, \states, \targetstates, \safestates, \directions[\outeraction], \directions[\inneraction],  \initstates, \reward, \detertrans)$ for which \Cref{assum:reach_avoid} holds is convex-incave.
% 
    \sdeni{}{Moreover, saddle-point-oracle gradient descent (\Cref{alg:oracle_sgda}) is guaranteed to converge in such games to recursive Stackelberg equilibrium policies in polynomial time.} \amy{wait, what!? you prove your theorems for convex-incave? i thought you hadn't bothered?}
\end{restatable}

==> fisher.tex <==
\section{Applications and Experiments}

if we re-define the follower's policy to be also a function of the action of the leader and restrict the follower to play only feasible actions given the leader's action such that $\policy[\inner]: \states \times \outeractions \to \coupledactions(\policy[\outer])$. This is also natural from a game perspective, since in a Stackelberg game, at each state $\state$ the follower observes the leader's action $\outeraction$ and then only plays a feasible action $\inneraction \in \coupledset(\state, \outeraction)$.


\subsection{Stochastic Fisher Markets}

A \mydef{(one-shot) Fisher market} consists of $\numbuyers$ buyers and $\numgoods$ divisible goods \cite{brainard2000compute}.
Each buyer $\buyer \in \buyers$ is endowed with a budget $\budget[\buyer] \in \budgetspace[\buyer] \subseteq \mathbb{R}_{+}$ and a utility function $\util[\buyer]: \mathbb{R}_{+}^{\numgoods} \times \typespace[\buyer] \to \mathbb{R}$, which is parameterized by a type $\type[\buyer] \in \typespace[\buyer]$ that defines a preference relation over the consumption space $\R^\numgoods_+$.
% \amy{you should introduce types here, if it is types that define utility functions!}
% \footnote{\sdeni{WLOG, we assume that all budgets are strictly positive; otherwise, we could remove a buyer with a zero budget without affecting the equilibrium.}{}} 
%As is standard in the literature, we assume that there is one divisible unit of each good in the market.
Each good is characterized by a supply $\supply[\good] \in \supplyspace[\good] \subset \R_+$.


An instance of a Fisher market is then a tuple $\calM \doteq (\numbuyers, \numgoods, \util, \type, \budget, \supply)$, $(\type, \budget, \supply)$ when $(\numbuyers, \numgoods, \util)$ are fixed and clear from context, where $\util = \left(\util[1], \hdots, \util[\numbuyers] \right)$ is a vector of utility functions, one per buyer, $\budget \in \R_{+}^{\numbuyers}$ is the vector of buyer budgets, and $\supply \in \R_{+}^{\numgoods}$ is the vector of supplies.

Given a Fisher market $(\type, \budget, \supply)$, an \mydef{allocation} $\allocation = \left(\allocation[1], \hdots, \allocation[\numbuyers] \right)^T \in \R_+^{\numbuyers \times \numgoods}$ is a map from goods to buyers, represented as a matrix, s.t. $\allocation[\buyer][\good] \ge 0$ denotes the amount of good $\good \in \goods$ allocated to buyer $\buyer \in \buyers$. Goods are assigned \mydef{prices} $\price = \left(\price[1], \hdots, \price[\numgoods] \right)^T \in \mathbb{R}_+^{\numgoods}$. A tuple $(\allocation^*, \price^*)$ is said to be a \mydef{competitive equilibrium (CE)} \cite{arrow-debreu, walras} if 
1.~buyers are utility maximizing, constrained by their budget, i.e., $\forall \buyer \in \buyers, \allocation[\buyer]^* \in \argmax_{\allocation[ ] : \allocation[ ] \cdot \price^* \leq \budget[\buyer]} \util[\buyer](\allocation[ ], \type[\buyer])$;
and 2.~the market clears, i.e., $\forall \good \in \goods,  \price[\good]^* > 0 \Rightarrow \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* = \supply[\good]$ and $\price[\good]^* = 0 \Rightarrow\sum_{\buyer \in \buyers} \allocation[\buyer][\good]^* \leq \supply[\good]$.

% \amy{move to appendix!}
%\samy{We denote the type space of all buyers $\typespace = \bigtimes_{\buyer \in \buyers} \typespace[\buyer]$, and the space of all possible budgets for all buyers $\budgetspace = \bigtimes_{\buyer \in \buyers} \budgetspace[\buyer]$. We denote the set of all goods' possible supplies $\supplyspace = \bigtimes_{\good \in \goods} \supplyspace[\good]$.}{}\deni{This should not be removed, it is used in the appendix, and is also our state space, it's important!}\amy{if it is not used in the main body, just define it in the appendix. if you want to use it here, it goes above the previous paragraph so you can then say $(t,b,q) \in T \times B \times Q$.}


A \mydef{stochastic Fisher market (with savings)} $\fishermkt[0] \doteq (\numbuyers, \numgoods, \util, \states, \initstates, \trans, \discount)$ is a market player over an infinite horizon $\iter = 1, 2, \hdots$ in which each state corresponds to a one-shot Fisher market: i.e., each state $\state \in \states = \typespace \times \budgetspace \times \supplyspace$ is characterized by a tuple $\state \doteq (\type, \budget, \supply)$.
The market is initialized at state $\staterv[0] \sim \initstates$, and for each state $\staterv[\iter] \doteq (\typerv[][\iter], \budgetrv[][\iter], \supplyrv[][\iter]) \in \states$ encountered at time step $\iter \in \N$, the market determines the prices $\price[][\iter]$ of the goods, while the buyers choose their allocations $\allocation[][][\iter]$ and set aside some \mydef{savings} $\saving[\buyer][\iter] \in [0, \budgetrv[\buyer][\iter]]$ to potentially spend at some future state.
Once allocations, savings, and prices have been determined, the market terminates with probability $1-\discount$, or it transitions to a new state $\staterv[\iter + 1] = \state^\prime$ with probability $\discount \trans(\state^\prime \mid \state, \saving)$, depending on the buyers' saving decisions.%
\footnote{In our model, which is consistent with the literature~\cite{romer2012advanced} 1.~prices do not determine the next state since market prices are set by a ``fictional auctioneer,'' not an actual market participant; 2.~allocations do not determine the next state.
Only savings, which are forward-looking decisions, affect future states---budgets, specifically.}
% We denote a stochastic Fisher market by $\fishermkt[0] \doteq (\numbuyers, \numgoods, \util, \states, \initstates, \trans, \discount)$.


% There exists two equivalent solution concepts for dynamic markets the sequential competitive equilibrium and the recursive competitive equilibrium. Suppose that $(\budget[][\iter], \type[][\iter], \supply[][\iter])_\iter$ is the sequence of states generated according to $\trans(\cdot \mid \state[\iter - 1], \allocation[][][\iter], \saving[][\iter])$ by  $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)},  {\price^*}^{(\iter)})_{\iter = 0}^\infty$. A \mydef{sequential competitive equilibrium} is a sequence of allocation, savings, and price tuples $({\allocation^*}^{(\iter)}, {\saving^*}^{(\iter)},  {\price^*}^{(\iter)})_{\iter = 0}^\infty$ such that 1) all buyers are expected utility maximizing constrained by their saving and spending constraints, i.e., for all  $\buyer \in \buyers$, 
% $
%     ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)})_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  (\allocation[\buyer][\iter]), \saving[\buyer][\iter]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq \budget[\buyer][\iter] + \saving[\buyer][\iter - 1] 
%     % \\ \budget[\buyer][\iter + 1] = \saving[\buyer][\iter]
%     }\right\}_{\iter = 1}^\infty } \sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer][][\iter], \type[\buyer][\iter])
% $ where $\type[\buyer][\iter]$, 
% and 2) The market clears in each time period 
% % \samy{and}{meaning}\deni{Not true, that would mean that goods unallocated are priced at zero only if Walras' law and feasibility holds.} 
% goods that are unallocated are priced at 0, i.e., for all $\good \in \goods$ and $\iter \in \N_+$,  if 
% $
%     {\price[\good]^*}^{(\iter)} > 0$ then $\sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = 1$, and if $
%     {\price[\good]^*}^{(\iter)} \geq 0$ then $\sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq 1
% $.

% % \mydef{sequential competitive equilibrium} which is sequence of allocation, saving and price tuples $({\allocation[][][\iter]}^*, {\saving[][\iter]}^* {\price[][\iter]}^*)_{\iter = 0}^\infty$ such that 1.~the buyers are expected utility maximizing constrained by the saving and spending constraint, i.e., for all $\buyer \in \buyers$, $ \{{\allocation[\buyer][][\iter]}^*, {\saving[][\iter]}^* \}_{\iter = 0}^\infty \in \argmax_{\left\{ \substack{  {\allocation[\buyer]^*}^{(\iter)} \in \R^{\numgoods}_+: \allocation[\buyer] \cdot {\price[][\iter]}^* + {\saving[][\iter]}^* \leq \budget[\buyer][\iter] }  \right\}_{\iter = 1}^\infty } \mathop{\E}_{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter])} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer](\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter])\right]$ 
% % % where $\state[\iter] = (\type[][\iter], \budget[][\iter], \supply[][\iter])$
% % 2.~the market clears in each time period and goods that are unallocated are priced at 0 in that state, i.e., for all $\good \in \goods$ and $\iter \in \N_+$, ${\price[\good]^*}^{(\iter)} > 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} = \supply[\good][\iter]$, or $ {\price[\good]^*}^{(\iter)} \geq 0 \implies \sum_{\buyer \in \buyers} {\allocation[\buyer][\good]^*}^{(\iter)} \leq \supply[\good][\iter]$. Unfortunately, although mathematically interesting, the sequential competitive equilibrium is untractable as it requires the computation of an infinite sequence.

% Note that the sequential competitive equilibrium allocations, savings, and prices at any time period are effectively a function of the state of the market, hence we could define a competitive equilibrium to be a mapping from states to a tuple of allocations, savings, and prices. Overloading notation, we define an \mydef{allocation policy}, $\allocation : \states \to \R_+^{\numbuyers \times \numgoods}$ as a mapping from states to allocations, a \mydef{saving policy} $\saving: \states \to \R_+^\numbuyers$ as a mapping from states to savings, and a \mydef{pricing policiy} $\price: \states \to \R_+^{\numgoods}$ as a mapping from states to prices.
% %




% Define $\budgetval[\buyer]: \states 
% % \times \R^{\states \times \numbuyers \times \numgoods} \times \R^{\states \times \numbuyers} \times \R^{\states \times \numgoods} 
% \to \R$ 
% % \deni{Add parameters to description}:
% \begin{align}
%     \budgetval[\buyer](\type, \budget, \supply
%     % ; \allocation, \saving, \price
%     ) &= 
%     % \max_{\left\{ \substack{  ({\allocation[\buyer]^*}^{(\iter)}, {\saving[\buyer]^*}^{(\iter)}) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot {\price^*}^{(\iter)} + \saving[\buyer][\iter] \leq (1+\interest)\saving[\buyer][\iter -1] + \budgetrv[\buyer][\iter] }  \right\}_\iter }
%     \mathop{\E}_{\substack{\state[\iter+1] \sim \trans(\cdot \mid \state[\iter], \allocation[][][\iter], \saving[][\iter])\\ \state[0] = \state }} \left[\sum_{\iter = 0}^\infty \discount^\iter \util[\buyer]\left(\allocation[\buyer]^{(\iter)}; \type[\buyer][\iter]\right)\right]\\
%     &= \util[\buyer]\left(\allocation[\buyer](\type, \budget, \supply), \type[\buyer]\right) + \mathop{\E}_{\state^\prime \sim \trans(\cdot \mid \state, \allocation[][][](\state), \saving[][](\state)) } \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + (1+\interest) \saving(\type, \budget, \supply), \supply^\prime; \allocation, \saving, \price) \right]
% \end{align}

% We can then re-express a sequential competitive equilibrium as a recursive competitive equilibrium.

Given a stochastic Fisher market with savings $\fishermkt[0]$
%$(\states, \util, \state[0], \trans, \discount)$, 
a \mydef{recursive competitive equilibrium (recCE)} \cite{mehra1977recursive} is a tuple $(\allocation^*, \saving^*, \price^*) \in \R_+^{\numbuyers \times \numgoods \times \states} \times \R_+^{\numbuyers \times \states} \times \R_+^{\numgoods \times \states}$, which consists of stationary \mydef{allocation}, \mydef{savings}, and \mydef{pricing policies} s.t.\ 1) the buyers are expected utility maximizers, constrained by their savings and spending constraints, i.e., for all buyers $\buyer \in \buyers$, $(\allocation[\buyer]^*, \saving[\buyer]^*)$ is an optimal policy that, for all states $\state \doteq (\type, \budget, \supply) \in \states$, solves the \mydef{consumption-savings problem}, defined by the following Bellman equations: for all $\state \in \states$, $\budgetval[\buyer](\state) =$
$$
    %\budgetval[\buyer](\type, \budget, \supply) =
    \max_{(\allocation[\buyer], \saving[\buyer]) \in \R^{\numgoods + 1}_+: \allocation[\buyer] \cdot \price^*(\state) + \saving[\buyer] \leq \budget[\buyer]} \left\{ \util[\buyer]\left(\allocation[\buyer], \type[\buyer]\right) 
    % \\ \notag   & 
    + \discount \mathop{\Ex}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \state, (\allocation[\buyer], \allocation_{-\buyer}^*(\state)), (\saving[\buyer], \saving_{-\buyer}^*(\state)))} \left[ \budgetval[\buyer](\type^\prime, \budget^\prime + \saving[\buyer], \supply^\prime) \right] \right\},
$$ 
%for all states $(\type, \budget, \supply) \in \states$ 
where $\allocation^*_{-\buyer}$, $\saving^*_{-\buyer}$ denote the 
%competitive equilibrium 
allocation and saving policies excluding buyer $\buyer$; and
2) the market clears in each state so that unallocated goods in each state are priced at 0, i.e., for all $\good \in \goods$ and $\state \in \states$,
$    
        \price[\good]^*(\state) > 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\state) = \supply[\good]
$ and
$
        \price[\good]^*(\state) \geq 0 \implies \sum_{\buyer \in \buyers} \allocation[\buyer][\good]^*(\state) \leq \supply[\good]
$.
% \samy{By analogy with Markov perfect equilibrium, we can view a}
A recCE is Markov perfect, as it is a CE regardless of initial  state,%
\footnote{Just as any stochastic game can be (non-compactly) represented as a one-shot game, any stochastic Fisher market with savings can be represented as a one-shot Fisher market comprising the same buyers (with utility functions given by their discounted cumulative expected utility) 
% $\Ex_{\staterv[\iter]} \left[\discount^\iter \util[\buyer]\left(\allocation[\buyer][][\iter], \type[\buyer][][\iter]\right) \right]$
\samy{}{and the same goods\deni{saying the same goods is confusing because in the new market you think of the goods at each time step as being seperate good, I like the previous version better.}, enhanced with time-stamps.}
It has been shown that competitive equilibria exist in such markets\cite{prescott1972note}.
In particular, a recCE is a CE in this market; the time stamps ensure that the market clears at every time step, as required.}
%\amy{does whoever writes about the time-stamped construction prove that CE exist in these one-shot markets? also, would a recursive CE of the stochastic Fisher market also be a CE of this one-shot market?}
i.e., buyers are allocated expected discounted cumulative utility-maximizing goods regardless of initial state, and the aggregate demand for each good is equal to its aggregate supply \emph{at all states}.
\amy{why does the qualifier ``starting from any state'', or ``regardless of initial conditions'' apply only to the first half of this sentence and not the second?}\deni{Because the market clearance condition is more robust and holds in every time period. this is because the seller is myopic at recCE; only the buyers are long-term optimizers.}

The following theorem proven by \citeauthor{goktas2022zero} \cite{goktas2022zero} shows that we can build a zero-sum stochastic Stackelberg game whose \recSE{} correspond to the set of recCE of any stochastic Fisher market with savings.
% Since \recSE{} are guaranteed to exist, recCE are also guaranteed to exist.
As \recSE, and hence recCE, are independent of the initial market state, we 
denote stochastic Fisher markets with savings by $\fishermkt \doteq (\numbuyers, \numgoods, \util, \states, \trans, \discount)$.

\begin{restatable}{theorem}{thmfishermarketrecursiveeqm}
\label{thm:fisher_market_recursive_eqm}
A stochastic Fisher market with savings $\fishermkt$
in which $\util$ is a set of continuous and homogeneous utility functions and the transition function is continuous in $\saving[\buyer]$ has at least one recCE.
Further, the \recSE{}
that solves the following Bellman equations corresponds to a recCE of $\fishermkt$: 
\begin{align} \label{eq:fisher_bellman}
    \forall \state \in \states, \statevalue[][](\state) = \min_{\price \in \R_+^\numgoods} \max_{(\allocation, \saving) \in \R_+^{\numbuyers \times (\numgoods + 1)} : \allocation \price + \saving \leq \budget} \sum_{\good \in \goods} \supply[\good] \price[\good] 
    + \sum_{\buyer \in \buyers} \left(\budget[\buyer] - \saving[\buyer]\right) \log(\util[\buyer](\allocation[\buyer], \type[\buyer])) \notag\\ 
    + \discount \mathop{\Ex}_{(\type^\prime, \budget^\prime, \supply^\prime) \sim \trans(\cdot \mid \state, 
    % \allocation, 
    \saving)} \left[\statevalue[][](\type^\prime, \budget^\prime + \saving, \supply^\prime) \right]
\end{align} 
\end{restatable}


==> old_intro.tex <==
%%% MIN-MAX GAMES
Min-max optimization problems are ubiquitous.
They have been used to model a variety of problems across a range of fields, including generative adversarial networks (GANs) \cite{goodfellow2014gan}, statistical learning \cite{xu2009robustness, shafieezadeh2015distributionally, dai2019kernel}, online learning \cite{cesa2006prediction}, deep learning \cite{sinha2017certifiable, sinha2020certifying}, distributed computing \cite{shamma2008cooperative, mateos2010distributed}, fairness in machine learning \cite{dai2019kernel, edwards2016censoring, madras2018learning, sattigeri2018fairness, xu2018fairgan}, and generative adversarial imitation learning \cite{cai2019global, hamedani2018iteration}.
%
In such problems, the goal is to minimize a continuous function $\obj: \R^\outerdim \times \R^\innerdim \to \R$ along one dimension $\outer$, and maximize it along another dimension $\inner$, over respective non-empty and compact constraint spaces $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$, i.e., $\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner)$.
%
\amy{game interpretation. convex-concave. a minimax theorem holds (add assumptions), so the canonical solution is Nash.}

%%% STACKELBERG GAMES
More recently, the literature has turned its attention to solving min-max optimization problems with coupled constraints \cite{goktas2021minmax, tsaknakis2021minimax, zhang2022stackelbergminmax, dai2022stackelbergminmax, lu2023stackelbergminmax} in which the choice of $\outer$ determines the constraint space of $\inner$ via a constraint correspondence $\coupledset: \R^\outerdim \rightrightarrows \innerset \subset \R^\innerdim$: i.e., $\min_{\outer \in \outerset} \max_{\inner \in \coupledset(\outer)} \obj(\outer, \inner)$.
Because a minimax theorem does not hold for coupled constrained min-max optimization problems even when $\obj$ is convex-concave and $\coupledset$ is convex, \citet{goktas2021minmax} suggest that such optimization problems are best interpreted as a two-player sequential, i.e., \mydef{Stackelberg}, games, where the $\outer$-player, also called the leader, first commits to an action $\outerpoint \in \outerset$, after which the $\inner$-player, also called the follower, having observed the leader's action, makes her move $\innerpoint(\outerpoint) \in \coupledset(\outerpoint)$.
% $\left\{\inner \in \innerset \mid (\outer, \inner) \in \coupledset \right\}$. 
The solution to a 
%min-max optimization problem with coupled constraints---hereafter 
min-max Stackelberg game can then be interpreted as a Stackelberg equilibrium, i.e., a tuple $(\outer[][][*], \inner[][][*]) \in \coupledset$, s.t.\ $\outer[][][*]$ maximizes $\obj$ over $\outerset$ assuming the follower will best respond to the leader's choice, whatever it happens to be, i.e., given any action $\outer[][][]$ for the leader, the follower will choose an action $\inner[][][*] (\outer[][][])$ that maximizes $\otherobj(\outer, \cdot)$ over $\innerset$, so that $\inner[][][*]$ is a best response to $\outer[][][*]$.
%%% EXISTENCE
%Here, to ensure existence, it is assumed that the constraint set $\outerset$ is non-empty and compact, and the constraint correspondence $\coupledset$ is continuous (i.e., upper and lower hemicontinuous), non-empty, and compact-valued.

\citeauthor{goktas2021minmax} (\citeyear{goktas2021minmax}) analyzed 
convex-concave min-max Stackelberg games, i.e., min-max Stackelberg games in which $\outerset$ is convex, $\coupledset$ is convex-valued, the marginal function $\val(\outer) \doteq \max_{\inner \in \coupledset(\outer)} \obj(\outer, \inner)$ is convex, and for all $\outer \in \outerset$, $\obj(\outer, \inner)$ is concave in $\inner$. 
A sufficient condition to ensure that a min-max Stackelberg game is convex-concave is for $\outerset$ to be convex, $\coupledset$ to be convex-valued and concave, i.e. for all $\lambda \in (0,1), \outer, \outer[][][\prime] \in \outerset$, $\coupledset(\lambda \outer + (1-\lambda) \outer[][][\prime]) \subseteq \lambda \coupledset(\outer) + (1-\lambda) \coupledset(\outer[][][\prime])$,%
\footnote{See Chapter 36 of \citeauthor{czerwik2002functional} (\citeyear{czerwik2002functional}) for a comprehensive review of concave correspondences.}
and $\obj$ to be convex in $(\outer, \inner)$ and concave in $\inner$. 
\citeauthor{goktas2021minmax} showed that, in such games, a Stackelberg equilibrium can be computed in polynomial time via nested gradient descent ascent, assuming access to an exact first-order oracle which provides the gradient of the objective and constraints\deni{Might need to be more careful here}.
Convex-concave min-max Stackelberg games have found applications in economics \cite{goktas2021minmax}, automated test generation \cite{badithela2022synthesizing}, and the design of autonomous vehicle safety concepts \cite{leung2022learning}.

% with $\innerset$ convex and $\coupledset$ strictly convex.%
% \footnote{We note that the strict convexity assumption can be relaxed to convexity if one instead assumes that the interior of $\coupledset$ is non-empty.}

% Define the \mydef{marginal function}%
% \footnote{\citet{goktas2021minmax} use the value function terminology to refer to the marginal function but we reserve this terminology for Markov Stackelberg games in this paper.} 
% $\val(\outer) \doteq \max_{\inner \in \innerset: (\outer, \inner) \in \coupledset} \obj(\outer, \inner)$.

%%% STOCHASTIC
In a \mydef{stochastic} min-max optimization problem, one is given a stochastic objective function $\objrv[\obji]: \R^\outerdim \times \R^\innerdim \to \R$, and the intent is to respectively minimize and maximize along the first and second dimensions for respective constraint spaces $\outerset \subset \R^\outerdim$ and $\innerset \subset \R^\innerdim$, in expectation over a distribution $\objdistrib \in \simplex(\objs)$ of parameters $\objs$, i.e., $\min_{\outer \in \outerset} \max_{\inner \in \innerset} \obj(\outer, \inner) \doteq \Ex_{\obji \sim \objdistrib} \left[ \obj[\obji](\outer, \inner) \right] .$
% , defining for each parameter $\obji \in \objs$, an \mydef{objective function} $\obj[\obji]: \R^\outerdim \times \R^\innerdim \to \R$
It is assumed that for all parameters $\obji \in \objs$, the objective function $\obj[\obji]$ is continuous. 
\amy{The object of study in this paper: we assume both stochasticity and coupled constraints...}
$\min_{\outer \in \outerset} \max_{\inner \in \coupledset(\outer)} \obj(\outer, \inner) \doteq \Ex_{\obji \sim \objdistrib} \left[ \obj[\obji](\outer, \inner) \right]$,


==> pacman.tex <==
\if 0
%%% PAC-MAN as a Stackelberg game
In the example of Pac-Man, we can model the ghosts collectively as the leader and Pac-Mac as the follower of a zero-sum stochastic Stackelberg game, where the action space of the ghost are any location in the maze, the action correspondence of Pac-Man outputs all locations in the that are not occupied by the ghost and the rewards are at each state is 1 if Pac-Man ate a pellet at that state and 0 otherwise. In this Stackelberg game, Pac-Man first observes the direction towards which the ghost will head, and then based on the paths that were blocked in the maze decide what direction to take, so as to avoid getting caught.%
\footnote{Alternatively, one might initially consider modelling the problem of training a Pac-Man agent as a stochastic generalized Nash equilibrium problem \cite{franci2021stochastic} to ensure safety, however, at a generalized Nash equilibrium both players can constrain one another's actions, this would be an incorrect model of Pac-Man since the ghost are choices are not constrained by Pac-Man.} \deni{Need to add something on why modelling pac-man as a zero-sum stochastic game would be for safety even if you penalize actions that get him caught.} This then allows Pac-Man to avoid getting into a situation where it can get caught and hence lose the game.
\fi

Pac-Man is a video game in which the protaganist moves through a maze trying to eat all the pellets, while being chased by a group of antagonists, the ghosts, whose movements restrict the paths that Pac-Man can take.
%%%often forcing him
%\footnote{\samy{}{It is worth noting that the characters in Pac-Man, perhaps \emph{the\/} most popular video game of all time, were explicitly designed to appeal to girls and women.} \deni{I would have never thought that ngl} \amy{couldn't help myself!}}
%%%to change direction. 
As a reach-avoid problem, Pac-man is naturally modeled as a two-player zero-sum (Stackelberg) game with the team of ghosts as the defender and Pac-man as the attacker.
%The game ends when the attacker reaches a target, but when rewards are discounted, the attacker is incentivized to get there sooner rather than later.
Reach-avoid also characterizes the problems faced by self-driving cars, which aim to reach their destination without getting into an accident \cite{leung2022learning}.
%As such the autonomous car is assumed to be the attacker, while all other cars on the road are modelled as defenders \cite{zhou2018efficient, bansal2017hamilton}.
%In this setting, we assume worst-case behavior from the other cars on the road, namely them trying to hit the autonomous car, since simple accidents can lead to loss of human life and ensuring safety is as a result paramount.
%Modeling the problem of training an autonomous car as a Stackelberg game in which the cars on the road are collectively the leader and the autonomous car is the follower can ensure that the autonomous car gets to its destination while avoiding maneuvers that could lead to a collision. 
Autonomous driving thus naturally lends itself to the formalism of zero-sum games \cite{zhou2018efficient, bansal2017hamilton}---but in particular, Stackelberg games: like the ghosts in Pac-man, the other cars on the road can be viewed collectively as the leader/defender, while the autonomous car, which aims to reach its destination without getting into an accident, is the follower/attacker. 


==> policy_envelope.tex <==

Additionally, consider for any fixed leader parameter $\outerpoint \in \outerset$, define the set of the optimal follower parameters $\inners^*(\outerpoint) \doteq \argmax_{\inner \in \innerset} \min_{\langmult \in \langmults} \lang(\inner, \langmult; \outerpoint) $ and the KKT multipliers associated with them $\langmults^*(\outerpoint, \inner[][][*](\outerpoint)) \doteq \argmin_{\langmult \in \langmults} \lang(\inner[][][*](\outerpoint), \langmult; \outerpoint)$. The \mydef{policy envelope theorem} tells us the gradient of the marginal function of the game at any leader parameter $\outerpoint \in \outerset$ is equal to the gradient of the game Lagrangian w.r.t. the follower parameter $\outer$ evaluated at $\outerpoint$, the best-response policy parameter $\inner[][][*](\outerpoint)$ of the follower, and the associated Lagrange multipliers $\langmult[][*](\outerpoint)$

\begin{theorem}[Policy Envelope Theorem]
Consider the zero-sum stochastic Stackelberg game $\initgame$. 
% Suppose that \ref{assum:follower_zero} holds.
Then, the gradient of the marginal function $\marginalfunc(\outer) = \max_{\inner \in \innerset : \constr(\policy[\outer], \policy[\inner]) \geq \zeros} \cumulutil(\outer, \inner)$ w.r.t. $\outer$ at $\outerpoint \in \outerset$, if it exists is given by:
\begin{align}
    \grad[\outer] \marginalfunc(\outer) = 
    \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    }  \left[\grad[\outeraction] \actionvalue[][{(\outerpoint, {\inner[][][*](\outerpoint)})}](\staterv, \policy[\outerpoint](\staterv), \policy[{\inner[][][*](\outerpoint)}](\staterv))  \grad[\outer] \policy[\outerpoint](\staterv) \right] + \left< \policy[\langmult], \constr[](\policy[\outer], \policy[\inner]) \right>
    % \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    % }  \left[\lang[\state]({\inner[][][*](\outerpoint)}, \langmult[][*](\outerpoint); \outerpoint) \right]
\end{align}
where ${\inner[][][*](\outerpoint)} \in \inners^*(\outerpoint) = \argmax_{\inner \in \innerset} \min_{\langmult \in \langmults} \lang(\inner, \langmult; \outer)$ and ${\langmult[][*](\outerpoint, \inner[][][*](\outerpoint)) } \in \langmults^*(\outerpoint, \inner[][][*](\outerpoint)) = \argmin_{\langmult \in \langmults}  \lang(\inner[][][*](\outerpoint), \langmult; \outerpoint)$.
\end{theorem}

More generally, guaranteeing the differentiability of the marginal function of the game can be too restrictive as this requires the optimal solution to the saddle point problem $\max_{\inner \in \innerset} \min_{\langmult \in \langmults} \lang(\inner, \langmult; \outer)$ which can only be ensured by assuming strict convexity in $\inner$ and restrictive constraint qualifications such as the strict Mangasarian-Fromovitz constraint qualification. However, we can guarantee the convexity of the marginal function under the following assumption, and in aim to to characterize the set of subdifferentials of the marginal function.

\begin{assumption}[Leader Assumptions]\label{assum:leader_zero}
    Consider the zero-sum stochastic Stackelberg game $\initgame$ and the leader's policy function $\policy[\outer]$. Suppose that for all states $\state \in \states$, 1.~ $\reward(\state, \outeraction, \inneraction), \constr[][1](\state, \outeraction, \inneraction), \hdots, \constr[][\numconstrs](\state, \outeraction, \inneraction)$ is convex in $(\outeraction, \inneraction)$, 
    2.~ $\trans(\state^\prime \mid \state, \outeraction, \inneraction)$ is continuous and CSD convex in $\outeraction$ \deni{Figure out if we want convex in both}, and
    3.~$\outerset$ is non-empty, compact, and convex, and
    4.~ $\policy[\outer]$ is affine in $\outer$.
\end{assumption}

Since the marginal function is guaranteed to be convex under \Cref{assum:leader_zero}, its subdifferential is non-empty at all points of the domain of the marginal function. 

\begin{theorem}[Subdifferential Policy Envelope Theorem]
Consider the zero-sum stochastic Stackelberg game $\initgame$. Suppose that \ref{assum:follower_zero}, and \ref{assum:leader_zero} hold. 
% Additionally, assume that $\policy[\inner]$ is continuous and affine in $\outer$.
Then, the subdifferential of the marginal function $\marginalfunc(\outer) = \max_{\inner \in \innerset : \constr(\policy[\outer], \policy[\inner]) \geq \zeros} \cumulutil(\outer, \inner)$ w.r.t. $\outer$ at $\outerpoint \in \outerset$, if it exists is given by:
\begin{align}
    \grad[\outer] \marginalfunc(\outer) = 
    % \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    % }  \left[\grad[\outeraction] \actionvalue[][{(\outerpoint, {\inner[][][*](\outerpoint)})}](\staterv, \policy[\outerpoint](\staterv), \policy[{\inner[][][*](\outerpoint)}](\staterv))  \grad[\outer] \policy[\outerpoint](\staterv) + \sum_{\numconstr = 1}^\numconstrs \policy[{\langmult[][*](\outerpoint)}][][][\numconstr](\staterv) \grad[\outer]\left[\constr[][\numconstr](\state, \policy[\outer](\staterv), \policy[{\inner[][][*](\outerpoint)}](\staterv)) \right] \right]
     \mathrm{conv} \left( \bigcup_{\inner[][][*](\outerpoint) \in \innerset^*(\outerpoint)}      \bigcup_{\langmult[][*](\outerpoint, \inner[][][*](\outerpoint)) \in \langmults[\numconstr]^*(\outerpoint, \inner[][][*](\outerpoint))} \left\{ \mathop{\Ex}_{\staterv \sim \statedist[\initstates][{(\outerpoint, \innerpoint)}]
    % \\ \actionrv \sim \policy[\outer](\cdot \mid \staterv)}
    }  \left[\lang[\state]({\inner[][][*](\outerpoint)}, \langmult[][*](\outerpoint, \inner[][][*](\outerpoint)); \outerpoint) \right] \right\} \right)
\end{align}
where $\mathrm{conv}$ is the convex hull operator and $\inners^*(\outerpoint) = \argmax_{\inner \in \innerset} \min_{\langmult \in \langmults} \lang(\inner, \langmult; \outer)$ and $\langmults(\outerpoint, \inner[][][*](\outerpoint)) = \argmin_{\langmult \in \langmults}  \lang(\inner[][][*](\outerpoint), \langmult; \outerpoint)$ 
\end{theorem}


==> prelim_pseudogame.tex <==
\section{Preliminaries}

\subsection{Notation}
We use caligraphic uppercase letters to denote sets (e.g., $\calX$), bold uppercase letters to denote matrices (e.g., $\allocation$), bold lowercase letters to denote vectors (e.g., $\price$), lowercase letters to denote scalar quantities, (e.g., $x$), and uppercase letters to denote random variables (e.g., $X$).
We denote the $i$th row vector of a matrix (e.g., $\allocation$) by the corresponding bold lowercase letter with subscript $i$ (e.g., $\allocation[\buyer])$. 
Similarly, we denote the $j$th entry of a vector (e.g., $\price$ or $\allocation[\buyer]$) by the corresponding Roman lowercase letter with subscript $j$ (e.g., $\price[\good]$ or $\allocation[\buyer][\good]$).
We denote functions by a letter determined by the value of the function
e.g., $f$ if the mapping is scalar valued, $\f$ if the mapping is vector valued, and $\calF$ if the mapping is set-valued.
We denote the vector of ones of size $\numbuyers$ by $\ones[\numbuyers]$.
We denote the set of integers $\left\{1, \hdots, n\right\}$ by $[n]$, the set of natural numbers by $\N$, and the set of real numbers by $\R$. We denote the positive and strictly positive elements of a set by a $+$ and $++$ subscript respectively, e.g., $\R_+$ and $\R_{++}$. 
the set of positive natural numbers by $\N_+$ , the set of non-negative real numbers by $\R_+$, and the set of strictly positive real numbers by $\R_{++}$.
We denote the orthogonal projection operator onto a set $C$ by $\project[C]$, i.e., $\project[C](\x) = \argmin_{\y \in C} \left\|\x - \y \right\|_2^2$.
We denote by $\simplex[n] = \{\x \in \R_+^n \mid \sum_{i = 1}^n x_i = 1 \}$ the unit simplex in $\R^n$, and by $\simplex(A)$ the set of probability measures on the set $A$.
We define $\ball[\varepsilon][\x] = \{ \z \in \calZ \mid ||\z - \x || \leq \varepsilon \}$ to be the closed epsilon ball centered at $\x$; here $\calZ$ and $\|\cdot \|$ will be clear from context.
We denote the indicator function of a set $\calC$ by $\setindic[\calC](\x) = 0$ if $\x \in \calC$ and $\setindic[\calC](\x) = \infty$ if $\x \notin \calC$.
We abbreviate  $\mathop{\Ex}[f(\action) \mid \policy(\state)  = \action]$, the conditional expectation of $f(\action)$ for a given function $f$ with respect policy profile $\policy$ at a given state $\state$, by $\mathop{\Ex}^{\policy}[f(\action)]$.
Given two vector $\x, \y \in \R^n$, we write $\x \geq \y$ or $\x > \y$ to mean component-wise $\ge$ or $>$ respectively.

\deni{Space permitting, add something about how you separate a vector into two, i.e., the game theory notation.}
\deni{Consider doing away with the random variable notation.}


\subsection{Mathematical Preliminaries} 
Given $A \subset \R^\outerdim$, the function $\obj: \calA \to \R$ is said to be $\lipschitz[\obj]$-\mydef{Lipschitz-continuous}  w.r.t.\ norm $\left\| \cdot \right\|$ iff $\forall \outer_1, \outer_2 \in \calX, \left\| \obj(\outer_1) - \obj(\outer_2) \right\| \leq \lipschitz[\obj] \left\| \outer_1 - \outer_2 \right\|$.
% \deni{I think we are safe to remove also the next two paragraphs} A \mydef{variational inequality (VI)} problem $(\constraintset, \objs)$ given by a set $\constraintset$ and a function $\objs: \constraintset \to \R^\numconstrs$, consists of finding a solution $\x^* \in \constraintset$, $(\x - \x^*)^T \objs(\x^*) \geq 0.$ 
% We first show the following first order necessary and sufficient first order condition for a point to be a solution to a VI. 
A mapping $L : \calA \to \calB$ is said to be a \mydef{contraction mapping} (resp.\@ \mydef{non-expansion}) w.r.t.\ norm $\left\| \cdot \right\|$ iff it is $k$-lipschitz continuous w.r.t. norm $\left\| \cdot \right\|$ for $k \in [0,1)$ (resp.\@ $k = 1$).
% such that $\left\| L(\x) - L(\y) \right\| \leq k \left\| \x - \y \right\|$.

% A \mydef{quasi-variational inequality (QVI)} problem $(\constraints, \objs)$ given by a constraint correspondence $\constraints : \constraintset \to \constraintset$ and a function $\objs: \actionspace \to \R^\numactions$, consists of finding a solution $\x^* \in \constraintset$ such that $(\x - \x^*)^T \objs(\x^*) \geq 0$ for all $\x \in \constraints(\x^*)$. 

% % Finally, we define several concepts that are needed in our convergence proofs.
% Given $A \subset \R^\outerdim$, the function $\obj: \calA \to \R$ is said to be $\lipschitz[\obj]$-\mydef{Lipschitz-continuous} iff $\forall \outer_1, \outer_2 \in \calX, \left\| \obj(\outer_1) - \obj(\outer_2) \right\| \leq \lipschitz[\obj] \left\| \outer_1 - \outer_2 \right\|$.
% If the gradient of $\obj$, $\grad \obj$, is $\lipschitz[\grad \obj]$-Lipschitz-continuous, we then refer to $\obj$ as $\lipschitz[\grad \obj]$-\mydef{Lipschitz-smooth}.
% A function $\obj: \calX \to \R$ is $\mu$-\mydef{strongly convex (SC)} if $\obj(\outer_1) \geq \obj(\outer_2) + \left< \grad[\outer] \obj(\outer_2), \outer_1 - \outer_2 \right> + \nicefrac{\mu}{2} \left\| \outer_1 - \outer_1 \right\|^2$, and $\mu$-\mydef{strongly concave} if $-\obj$ is $\mu$-strongly convex. 


% A \mydef{min-max Stackelberg game}, denoted $(\outerset, \innerset, \obj, \constr)$, is a two-player, zero-sum game, where one player, who we call the $\outer$-player (resp.\ the $\inner$-player), is trying to minimize their loss (resp.\ maximize their gain), defined by a continuous \mydef{objective function} $\obj: X \times Y \rightarrow \mathbb{R}$, by choosing a strategy from a compact \mydef{strategy set} $\outerset \subset \R^\outerdim$ (resp. $\innerset \subset \R^\innerdim$), and  s.t.\ $\constr(\outer, \inner) \geq 0$ where $\constr(\outer, \inner) = \left(\constr[1] (\outer, \inner), \hdots, \constr[\numconstrs](\outer, \inner) \right)^T$ with $\constr[\numconstr]: \outerset \times \innerset \to \R$. A strategy profile $(\outer, \inner) \in \outerset \times \innerset$ is said to be \mydef{feasible} iff for all constraints $\numconstr \in [\numconstrs]$, $\constr[\numconstr] (\outer, \inner) \geq 0$.
% The function $\obj$ maps a pair of feasible strategies taken by the players $(\outer, \inner) \in \outerset \times \innerset$ to a real value (i.e., a payoff), which represents the loss (resp.\ the gain) of the $\outer$-player (resp.\ $\inner$-player).
% A min-max game is said to be convex-concave if the objective function $\obj$ is convex-concave. The relevant solution concept for Stackelberg games is the \mydef{Stackelberg equilibrium (SE)}. A strategy profile $\left(\outer^{*}, \inner^{*} \right) \in \outerset \times \innerset$ such that $\constr(\outer^{*}, \inner^{*}) \geq \zeros$ is a \mydef{Stackelberg equilibrium} if $\max_{\inner \in \innerset : \constr(\outer^{*}, \inner) \geq 0} \obj \left( \outer^{*}, \inner \right) \leq \obj \left( \outer^{*}, \inner^{*} \right) \leq \min_{\outer \in \outerset} \max_{\inner \in \innerset : \constr(\outer, \inner) \geq 0} \obj \left( \outer, \inner \right)$.

% \begin{definition}
% A strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ is a \mydef{local Stackelberg equilibrium} of $(\outerset, \innerset, \obj, \constr)$ if there exists $\varepsilon, \delta > 0$  such that:
% \begin{align}
%     \min_{\outer \in \outerset \cap \ball[\varepsilon][\outer]} \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer, \inner) \geq 0} \obj(\outer, \inner) \leq \obj(\outer^*, \inner^*) \leq \max_{\inner \in \innerset \cap \ball[\delta][\inner] : \constr(\outer^*, \inner) \geq 0} \obj(\outer^*, \inner)
% \end{align}
% \end{definition}
% A strategy profile $(\outer^*, \inner^*) \in \outerset \times \innerset$ is a \mydef{leader-local Stackelberg equilibrium} the above definition holds for $\delta = \infty$.

% % A \mydef{(normal-form) game} $(\numplayers, \actionspace, \util)$ consists of  $\numplayers \in \N_+$ players. Each player $\player \in \players$ is characterized by a set of non-empty, compact, and convex strategies $\actionspace[\player]$, and a continuous utility function $\util[\player]: \actionspace \to \R$ concave in $\action[\player] \in \actionspace[\player]$ for all $\naction[\player] \in \actionspace[-\player]$ where we denote the product strategy space of all players $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$ and the utility function for all players by $\util(\action) =  \left(\util[1](\action), \hdots, \util[\numplayers](\action) \right)^T$. A game $(\numplayers, \actionspace, \util)$ is said to be \mydef{monotone} if for all $\action, \otheraction \in \actionspace$,
% % $\sum_{\player \in \players} \left(\grad[{\action[\player]}] \util[\player](\action) - \grad[{\action[\player]}] \util[\player](\otheraction) \right)^T \left( \action - \otheraction \right) \leq 0$. A \mydef{Nash equilibrium (NE)} of a game $(\numplayers, \actionspace, \util)$ is a strategy profile $\action^* \in \actionspace$, i.e., a tuple of actions for each player, such that for all players $\player \in \players$, and for all $\action \neq \action^* \in \actionspace$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player]^*)$.


A \mydef{Markov decision process (MDP)} \cite{bellman1966dynamic} $\mdp \doteq  (\states, \actions, \reward, \trans, \discount, \initstates)$ is dynamic decision-making environment in which an agent starts in some state $\staterv[0] \sim \initstates \in \simplex(\states)$ taking actions that lead to rewards and transitions throughout the state space $\states$.
At each state $\state \in \states$ that the agent encounters, they take an action $\action \in \actions(\state)$ from their set of available actions, defined by the correspondence $\actions: \states \to \actionspace$.
% Players start the game at an initial state determined by an initial state distribution $\initstates: \states \to [0, 1]$ s.t.\ for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
After taking an action, the agent receives reward $\reward[ ]: \states \times \actionspace \to \R$, and the game either ends with probability $1-\discount$, where $\discount \in (0,1)$ is called the \mydef{discount factor}, or transitions to a new state $\state^\prime \in \states$, according to a \mydef{transition} probability function $\trans: \states \times \states \times \actionspace \to [0,1]$, where $\trans(\state^\prime \mid \state, \action) \in [0,1]$ denotes the probability of transitioning to state $\state^\prime \in \states$ from state $\state \in \states$ when action $\action \in \actions(\action)$ is taken.
We denote the space of all MDPs by $\mdps$.

The actions that the agent takes at each state can be described by a (stationary/Markovian) \mydef{policy}, i.e., a mapping from states to actions $\policy[ ]: \states \to \actionspace$, where $\policy(\state) \in \actionspace$ denotes the action taken by the agent at state $\state$.
A policy $\policy[ ]^*$ is \mydef{optimal} for an MDP $\mdp$ if  $\policy^* \in \argmax_{\policy} \mathop{\Ex}^{\policy}_{\substack{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \action[][][\iter]) \\ \staterv[0] \sim \initstates}} \left[ \sum_{\iter = 0}^\infty \discount^\iter \reward[ ](\staterv[\iter], \action[][][\iter]) \right]$: i.e., if the utility achieved by  $\policy^*$ exceeds that of all other policies.%
\footnote{In MDPs, it suffices to restrict attention to stationary/Markovian policies, as higher rewards cannot be attained~\cite{bellman1966dynamic}.}

% A \mydef{pseudo-game} $(\numplayers, \actions, \util)$ consists of $\numplayers \in \N_+$ player, with each player $\player \in \players$ trying to maximize their continuous payoff $\util[\player]: \actionspace \to \R$ which is concave in $\action[\player]$ by picking a feasible action from a set of actions $\actions[\player](\naction[\player]) \subseteq \actionspace[\player]$ determined by the actions $\naction[\player] \in \actionspace[-\player] \subset \R^\numactions$ of the other players, where $\actions[\player]: \actionspace[-\player] \rightrightarrows  \actionspace[\player]$ is a non-empty, compact, convex-valued, and continuous \mydef{action correspondence} which for convenience we represent as $\actions[\player](\naction[\player]) = \{ \action[\player] \in \actionspace[\player] \mid \actionconstr[\player][\numconstr](\action[\player], \naction[\player]) \geq \zeros, \forall \numconstr \in [\numconstrs]\} $. We denote the product of the feasible strategy correspondences of all player $\actions(\action) = \bigtimes_{\player \in \players} \actions[\player](\naction[\player])$. 
% A pseudo-game $(\numplayers, \actions, \util)$ is said to be \mydef{monotone} if for all $\action, \otheraction \in \actionspace$
% $\sum_{\player \in \players} \left(\grad[{\action[\player]}] \util[\player](\action) - \grad[{\action[\player]}] \util[\player](\otheraction) \right)^T \left( \action - \otheraction \right) \leq 0$. 
% A pseudo-game $(\numplayers, \actions, \util)$ is is said to have \mydef{jointly convex constraints} if the there exists $\constr: \actionspace \to \R^\numconstrs$ such that for all constraints $\numconstr \in [\numconstrs]$, $\constr[\numconstr](\action)$ is concave in $\action$, and we have $\constr = \actionconstr[1] = \hdots = \actionconstr[\numconstrs]$, in which case the joint strategy correspondence is simply a set, i.e., $\actions = \{\action  \in \actionspace \mid \constr(\action) \geq \zeros\}$. 

% % We define the \mydef{(logarithmic) Nash social welfare} $\nsw: \actionspace \to \R$ associated with a strategy profile $\action \in \actionspace$ by $\nsw(\action) = \sum_{\player \in \players} \log(\util[\player](\action))$ .

% A \mydef{generalized Nash equilibrium (GNE)} is a strategy profile $\action^*$ such that for all players $\player \in \players$, and $\action[\player] \in \actions[\player](\naction[\player]^*)$,  $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player]^*)$. A \mydef{variational equilibrium (VE) or normalized GNE} is a strategy profile $\action^*$ such that for all action profiles and $\action \in \actionspace$ such that $\actionconstr(\action) \geq \zeros$, $\util[\player](\action^*) \geq \util[\player](\action[\player], \naction[\player]^*)$. Note that although the set of VE of an pseudo-game is a subset of the set of GNE of the game, the converse is not true unless $\actionspace \subseteq \{\action \in \actionspace  \mid \actionconstr(\action) \geq \zeros\}$. 
% Note that although the set of VE of a pseudo-game is a subset of the set of GNE of the game, the converse is not true unless $\actionspace \subseteq \{\action \in \actionspace  \mid \actionconstr(\action) \geq \zeros\}$. 


% \deni{Assume rewards are positive for simplicity?}
An \mydef{(infinite horizon discounted) Markov pseudo-game} \cite{arrow-debreu,shubik1973fiat} $\game \doteq (\numplayers, \states, \actions, \reward, \trans, \discount, \initstates)$ is a dynamic $\numplayers$-player pseudo-game which is played over an infinite time horizon. The players start the game at time $\iter = 0$ in some state $\staterv[0] \sim \initstates \in \simplex(\states)$, and take simultaneous actions repeatedly, encountering a new state from a set of \mydef{states} $\states$ every time they take an action. 
% Players start the game at an initial state determined by an initial state distribution $\initstates: \states \to [0, 1]$ s.t.\ for all states $\state \in \states$, $\initstates(\state) \geq 0$ denotes the probability of the game being initialized at state $\state$.
At each time period $\iter = 0, 1, \hdots$, the players encounter a new state $\state[\iter] \in \states$, and each player $\player \in \players$ is constrained to play an action $\action[\player][][\iter] \in \actions[\player](\state[\iter], \naction[\player][][\iter])$ from a \mydef{(feasible) action correspondence} $\actions[\player]: \states \times \actionspace[-\player] \to \actionspace[\player]$, which defines the set of actions available to a player at state $\state[\iter]$, given the other players' actions $\naction[\player][][\iter]$ where we define $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$.
For convenience, we represent $\actions[\player](\state, \naction[\player]) = \{ \action[\player] \in \actionspace[\player] \mid (\action[\player], \naction[\player]) \in \actions(\state)\}$, where $\actions(\state)$ is the set of all \mydef{jointly feasible action profiles} at state $\state \in \states$.
%\sdeni{via functions $\actionconstr[\player][\numconstr](\state, \action[\player], \naction[\player])$,  concave in $\action[\player]$, for all constraints $\numconstr \in [\numconstrs]$.}{} 
% \sdeni{We define the joint action correspondence as $\actions(\state, \action) = \bigtimes_{\player \in \players} \actions[\player](\state, \naction[\player])$, \deni{I think we can remove this notation, don't see us using it anywhere!}\amy{is it even correct? why does $\actions$ depend on $\action$ and not $\action[-\player]$?}\deni{It is correct because it is the collection of all action profiles available to the players fixing all the players' strategies} and, as is standard in the literature, by abuse of notation
% where the set of all \mydef{jointly feasible action profiles} by $\actions(\state) = \{\action \in \actionspace \mid \actionconstr(\state, \action) \geq \zeros \}$.
% We further define $\actionspace = \bigtimes_{\player \in \players} \actionspace[\player]$.
% }{}

Once the players take their actions, each player $\player \in \players$ receives a \mydef{reward} $\reward[\player]: \state \times \actionspace \to \R$, and the game either ends with probability $1-\discount$, where $\discount \in (0,1)$ is called the \mydef{discount factor}, or transitions to a new state $\state^\prime \in \states$, according to a \mydef{transition} probability function $\trans: \states \times \states \times \actionspace \to [0,1]$, where $\trans(\state^\prime \mid \state, \action) \in [0,1]$ denotes the probability of transitioning to state $\state^\prime \in \states$ from state $\state \in \states$ when action profile $\action \in \actions(\action)$ is chosen by the players. 
A Markov pseudo-game is simply called a \mydef{Markov game} if, for all players $\player \in \players$, $\actions(\state, \naction[\player])$ is a constant correspondence for all $\state \in \states$, i.e., for all states $\state \in \states$, for all players $\player \in \players$, and for all strategy profiles $\action, \otheraction \in \actionspace[-\player], \actions(\state, \naction[\player]) = \actions(\state, \otheraction[-\player])$.
We can incorporate finite-action Markov pseudo-games with $d \in \N_+$ actions into this framework in the usual way, simply by taking the set of jointly feasible actions to be the probability simplex in  $\R^{\numplayers \times d}$: i.e., $\forall \state \in \states, \actions(\state) = \simplex[{d}]^\numplayers$.

%\deni{This is a technical point but in our definition we require the action correspondences to be continuous-set set valued as is standard in the literature}

% \deni{NOTE: in this paper we work only with joint policies which are deterministic in continuous action space and non-deterministic in discrete action spaces. So in discrete action spaces you have a distribution over outcomes.\amy{what's an outcome? a joint outcome?} 
% We note\amy{doesn't parse? please edit. e.g., ``do not''?} need anywhere in this paper marginal policies since we do note deal with eqm.}

% \deni{I think we should use either stationary/non-stationay or Markovian/non-Markovian but not both because in Markov games they coincide! I think we should remove stationary from our language and stick to Markovian since i think that is clearer... Either way non-Markovian includes non-stationary, but I do not think the inclusion holds the other way around. Since we look for non-markovian, and not non-stationary policies in this paper, we can scrap and referral to non-stationary etc...}
% \amy{i consulted chatGPT on this one:
% Amy: does non-Markovian imply non-stationary?
% ChatGPT: No, a process can be non-Markovian without being non-stationary, and vice versa. \\
% A non-Markovian process is one in which the future state of the process depends on not only the current state, but also on the past states. In other words, it violates the Markov property that the future state only depends on the current state. \\
% A non-stationary process is one in which the statistical properties of the process change over time. It means that the mean, variance, and other statistical properties of the process are dependent on the time index. \\
% So it is possible for a process to be non-Markovian and stationary, non-Markovian and non-stationary, Markovian and non-stationary, or Markovian and stationary. \\
% Amy, to Deni (i wouldn't want to hurt its feelings): of course, it doesn't really know what it is talking about, but it sure seems plausible! also, this is only about processes, not policies!}

A \mydef{stationary policy} for player $\player \in \players$, $\policy[\player]: \states \to \actionspace$ is a mapping from states to actions such that $\policy[\player](\state) \in \actionspace[\player]$ denotes the action player $\player$ takes at state $\state$. We denote \mydef{joint policies} $\policy = (\policy[1], \hdots, \policy[\numplayers]) : \states \to \actionspace$ such that $\policy(\action) \in \actionspace$ denotes the action profile played by the players at state $\state \in \states$. 
A \mydef{history of play} is a sequence of state-action tuples $\{(\state[\iter], \action[][][\iter])\}_{\iter} \subseteq (\states \times \actionspace)^{\N_+}$, which summarizes the states that have been observed throughout a Markov pseudo-game, and the actions taken at those states.
%\sdeni{Note that if the sequence is not an infinite one, then the game has not yet ended.}{}\amy{HUH? the game can end with some probability?}\deni{I do not remember writing this, and would like to think I have not!!!}
Then, a \mydef{(joint) non-Markovian  policy} \cite{maskin2001markov} $\policy: \states \times (\states \times \actionspace)^{\N_+} \to \actionspace$ is a mapping from states and histories of play to actions such that $\policy[\player](\state, \{(\state[\iter], \action[][][\iter])\}_{\iter} ) \in \actionspace[\player]$ denotes the action of player $\player$ at state $\state$, having observed the history of play $\{(\state[\iter], \action[][][\iter])\}_{\iter}$.
\sdeni{}{A policy $\policy \in \actionspace^\states$ is said to be \mydef{feasible} if, for all states $\state \in \states$, $\policy(\state) \in \actions(\state)$.}
We denote the set of all possible Markov pseudo-games by $\games$.

% \deni{TO REMOVE ENTIRELY}For simplicity,\amy{with or without LOG?} we focus on Markov pseudo-games with \mydef{joint constraints},%
% \footnote{We note that even in the static pseudo-game setting the majority of the literature to date has focused on pseudo-games with joint constraints; little is known beyond such games.}
% where for all players $\player, \otherplayer \in \players$ and constraints $\numconstr \in [\numconstrs]$, $\actionconstr[\player][\numconstr](\state, \action[\player], \naction[\player]) = \actionconstr[\otherplayer][\numconstr](\state, \action[\player], \naction[\player]) = \constr[\numconstr] (\state, \action)$, \samy{}{for some function $\constr$ s.t.\@ } \amy{or ``for some alternative set of constraints $\constr[\numconstr]$'', please finish!}. 
% When the constraints are joint, \samy{it}{the joint action correspondence} depends only on the states, i.e., $\actions(\state) = \left\{\action \in \actionspace \mid \constr(\state, \action) \geq 0 \right\}$\sdeni{,and is guaranteed to be non-empty, compact, and convex at all states}{}.\amy{why?}
% % introduce a function $\constrs : \actionspace^\states \to \R^{\numstates \times \numplayers \times \numconstrs}$ such that $\constrs(\policy) = (\constr(\state, \policy(\state))_{\state \in \states}$, and define feasible policy profiles as those $\policy \in  \actionspace^\states$ s.t.\ $\constrs(\policy) \geq \zeros$.

% \deni{Make this maybe only about the jointly constrained case?}\amy{seems like you did this?}


Given a Markov pseudo-game $\initgame$, the \mydef{state-value function} $\vfunc: \states \times \actionspace^\states \to \R^\numplayers$ and the \mydef{action-value function} $\qfunc: \states \times \actions \times \actions^\states \to \R^\numplayers$ are respectively defined as
% \begin{align}
$\vfunc[\player](\state; \policy) =$
$$
\mathop{\Ex^{\policy}}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \action[][][\iter])} \left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \action[][][\iter]) \mid
    % \outerrv[\iter] = \policy[\outer]( \staterv[\iter]), \innerrv[\iter]  = \policy[\inner](\staterv[\iter]),
    \staterv[0] = \state \right] %\label{eq:state_value}
$$
and $\qfunc[\player](\state, \action; \policy) =$
$$ 
     \mathop{\Ex^{\policy}}_{\staterv[\iter+1] \sim \trans( \cdot \mid \staterv[\iter], \action[][][\iter])}\left[\sum_{\iter = 0}^\infty \discount^\iter \reward[\player](\staterv[\iter], \action[][][\iter]) \mid \staterv[0] = \state, \action[][][0] = \action \right] \enspace ,
$$
for all $\player \in \players$.
The \mydef{ utility function} $\util[\player]: \actionspace^\states \to \R$ for a player $\player \in \players$, given policy profile $\policy$, is then defined as the player's expected cumulative  reward: i.e., $\util[\player](\policy) = \Ex_{\state \sim \initstates} [\vfunc[\player](\state; \policy)]$.


Given a Markov pseudo-game $\pgame$, we define the \mydef{regret} for player $\player \in \players$ for policy $\policy[\player]$ as compared to another policy $\otherpolicy[\player]$, given the policy profile $\policy[-\player]$ of other players, as 
%
%\begin{align}
    $\regret[\player][\pgame](\policy[\player], \otherpolicy[\player]; \policy[-\player]) = \util[\player][][\pgame](\otherpolicy[\player], \policy[-\player]) - \util[\player][][\pgame](\policy[\player], \policy[-\player])$.
Additionally, the \mydef{cumulative regret}, $\cumulregret[][\pgame]: \actionspace^\states \times \actionspace^\states \to \R$
between two policy profiles $\policy \in \actionspace^\states$ and $\otherpolicy \in \actionspace^\states$
%across all players in a pseudo-game $\pgame \in \pgames$ is 
is given by $\cumulregret(\otherpolicy; \policy) = \sum_{\player \in \players} \regret[\player][\pgame](\policy[\player], \otherpolicy[\player]; \policy[-\player])$.
%\enspace .
%\end{align}
%\noindent
% For notational simplicity, we will often write $\regret[\player][\pgame](\action[\player], \naction[\player]) = \max_{\otheraction[\player] \in \actions[\player](\naction[\player][][][*])} \util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])$
Further, the \mydef{exploitability}  (or \mydef{Niakido-Isoda potential  function} \cite{nikaido1955note}),
$\exploit[][\pgame]: \actionspace^\states \to \R$, of a policy profile $\action$ is defined as 
$\exploit[][\pgame](\policy) =  \sum_{\player \in \players} \max_{\otherpolicy[\player] \in \actions[\player](\naction[\player])} \regret[\player][\pgame](\action[\player], \otheraction[\player]; \naction[\player])$.
%An alternative name for exploitability in the GNE literature is the Nikaido-Isoda potential function
The max is taken over $\actions[\player](\naction[\player])$,
%to obtain the sum of unilateral deviations, 
since a player can only deviate within the set of feasible strategies. Note that an action profile $\action^*$ is a GNE iff $\exploit[][\pgame](\action^*) = 0$.

==> reach_avoid_old.tex <==
\label{sec_app:experiments}

%\sarjun{To compare the performance of the Stackelberg equilibrium, we also consider a zero-sum (simultaneous-move) stochastic game version of our reach avoid-game with the same state, action spaces and displacement function. In contrast, in this game to ensure that the attacker does not get caught by the defender we penalize the attacker when it gets into the safety radius of the defender. That is, since the attacker tries to reach a goal within a $g$ radius while staying out of a $c$ capture radius , leading to the following rewards:}{}

% \sarjun{}{TODO: fix the conditions, some of the targets should be fail states}

% % \sarjun{}{old}
% % \begin{align}
% %     \reward(\state, \outeraction[ ][ ], \inneraction[ ][ ]) = \begin{cases}
% %         1 & ||[x_1,y_1]^T_{\inneraction[ ][ ]} - [x_{\mathrm{goal}}, y_{\mathrm{goal}}]||_2  \leq g \\
% %         -1 & ||[x_1,y_1]^T_{\inneraction[ ][ ]} - [x_1,y_1]^T_{\outeraction[ ][ ]}||_2 \leq c \\ 0 & o.w.
% %     \end{cases}
% % \end{align} 
% % \sarjun{}{new}

% \sarjun{}{The reward function of the game is defined by \Cref{eq:stackelberg_reward} and trained with \Cref{alg:nested_pgda}.}

% \begin{equation}
% \reward(\state, \outeraction, \inneraction)  =
%     \begin{cases}
%          -\left\| {\state[][\inneraction]}^\prime - \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \right\|^2, &\detertrans[\inneraction](\state[][\inneraction],  \inneraction) \notin \targetstates, {\state[][\inneraction]}^\prime \in \targetstates \\
%         100, & \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \in \targetstates,{\state[][\inneraction]}^\prime \in \targetstates
%     \end{cases}
% \label{eq:stackelberg_reward}
% \end{equation} 

% \sarjun{}{To compare the performance of the Stackelberg equilibrium, we also consider a zero-sum simultaneous move stochastic version of our reach-avoid game with the same state, action spaces and displacement function. Importantly, we change the learning algorithm to trained with \Cref{alg:sim_pgda} and reward function so that the constraint correspondence is no longer enforced. Instead, we apply a penalty to the attacker if it is caught shown in \Cref{eq:nash_reward}}

% \begin{equation}
% \reward(\state, \outeraction, \inneraction)  =
%     \begin{cases}
%          -\left\| {\state[][\inneraction]}^\prime - \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \right\|^2, &\detertrans[\inneraction](\state[][\inneraction],  \inneraction) \notin \targetstates, {\state[][\inneraction]}^\prime \in \targetstates \\
%         100, & \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \in \targetstates,{\state[][\inneraction]}^\prime \in \targetstates \\
%         -100, & \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \in \targetstates,{\state[][\inneraction]}^\prime \in \calP + \detertrans[\outeraction] (\state, \outeraction)\
%     \end{cases}
% \label{eq:nash_reward}
% \end{equation} 

% \sarjun{}{Finally, we also implement a pursuit-evasion style variant of our game. In this case, we change the role of players from attacker and defender to pursuer and evader. In this case there is no target and the pursuer aims to mimimize the distance between itself and the defender. Since the constraint correspondence isn't needed for this varient we use the simultaneous version of our game with \Cref{alg:sim_pgda} and the following reward function.}

% \begin{equation}
% \reward(\state, \outeraction, \inneraction)  =
%     \begin{cases}
%          -\left\| {\state[][\inneraction]} - \state[][\outeraction] \right\|^2, 
%     \end{cases}
% \label{eq:pe_reward}
% \end{equation}

% \begin{equation}
% \reward(\state, \outeraction, \inneraction) =
%     \begin{cases}
%         100, & \left\| \detertrans[\outeraction](\state[][\outeraction],  \outeraction)  - \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \right\|^2 < \calP \\
%          - \left\| \detertrans[\outeraction](\state[][\outeraction],  \outeraction)  - \detertrans[\inneraction](\state[][\inneraction],  \inneraction) \right\|^2, & \text{ o.w.}
%     \end{cases}
% \label{eq:pe_reward}
% \end{equation} 

%\section{Experimental Results}

% \begin{figure}[htpb]
%   \centering
%     \includegraphics[width=\textwidth/2]{figures/training.png}
%   \caption{Running average of the outcome of the game across training episode. We can see that in the Stackelberg variant (lighter shading), the attacker (blue) performs comparably to the the Nash variant, however, the defender (red) wins much less often.}
%   \label{fig:training}
% \end{figure}

% \begin{table}[h]
% \centering
% \caption{Game Outcomes}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \textbf{Game} & \textbf{Attacker Wins} & \textbf{Defender Wins} & \textbf{Draws} & \textbf{Attacker Doesn't Lose} \\ \hline\hline
% Stackelberg & 493 & 34 & 473 & 966 \\ \hline
% Nash & 435 & 166 & 399 & 834 \\ \hline
% \end{tabular}
% \label{tab:game_outcomes}
% \end{table}

%\sarjun{Our results in \Cref{fig:training} show that the Stackelberg variant outperforms the Nash baseline during training. In particular, the rate of attacker wins is comparable, at around 30\% while the number of defender wins is much lower at around 20\% compared to the Nash rate of around 25\%. This shows that the Stackelberg variant is relatively safer since the attacker loses significantly less often, while maintaining a comparable win rate. The peaks and valleys in the win rate of the attacker is an interesting feature of \Cref{alg:nested_pgda}, since the alternating nature of the algorithm means that one player improves as the other is fixed. The Nash variant remains relatively flat as both players are updated simultaneously.  Nevertheless, the defender win-rate of the Nash baseline stays consistently below the Stackelberg counterpart. We also run the final trained attackers against a random defender for 1000 episodes, shown in \Cref{tab:game_outcomes} and find that the Stackelberg agent outperforms the Nash agent in both wins and draws.}{}

\subsection{Round Robin Tournament}
\amy{i think these results are redundant, so can be commented out?}

\begin{table}[H]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Scenario & Attacker Wins & Defender Wins & Draws \\ \hline
Stackelberg attacker vs Nash defender & $42.20 \pm 1.47$ & $6.80 \pm 1.33$ & $1.00 \pm 0.63$ \\ \hline
Stackelberg attacker vs Reverse defender & $50.00 \pm 0.00$ & $0.00 \pm 0.00$ & $0.00 \pm 0.00$ \\ \hline
Stackelberg attacker vs Stackelberg defender & $49.20 \pm 0.75$ & $0.80 \pm 0.75$ & $0.00 \pm 0.00$ \\ \hline
Nash attacker vs Nash defender & $30.40 \pm 2.15$ & $0.80 \pm 0.40$ & $18.80 \pm 1.94$ \\ \hline
Nash attacker vs Reverse defender & $0.00 \pm 0.00$ & $49.40 \pm 0.80$ & $0.60 \pm 0.80$ \\ \hline
Nash attacker vs Stackelberg defender & $9.60 \pm 3.38$ & $37.40 \pm 2.42$ & $3.00 \pm 1.67$ \\ \hline
\end{tabular}
\caption{Mean and standard deviation of results for each scenario.}
\end{table}

\arjun{In the Nash version of the game, both players are trained concurrently with no constraints imposed. we keep the same reward function as \Cref{sec_app:experiments}. However, this was after considering other reward functions that did not converge. In the reverse version of the game we switch the order of the attacker and the defender, such that the attacker becomes the leader and the defender becomes the follower. We also change the reward function such that the defender tries to minimize the distance between itself and the the attacker. This subtle change turns the reach-avoid into pursuit-evasion \cite{zhou2018efficient}. This results in quite different behaviour from the defender. In the normal Stackelberg case, the defender tries to block the attacker from reaching the goal, however in the reverse case, the defender is more aggressive and tries to crash into the attacker. Nevertheless, \Cref{fig:wins} shows that the Stackelberg attacker is robust to these changes in defender policy.}


==> stackelberg.tex <==

The \mydef{deterministic policy gradient theorem} \cite{silver2014deterministic}, generalizes the policy gradient theorem \cite{sutton1999policy} for deterministic policies, and provides us conditions under which the cumulative utility function of the game is differentiable w.r.t. to the parameters of the leader and follower's policies respectively:
\begin{align}
    \grad[\outer] \cumulutil(\outer, \inner) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\initstates][\policy]\\ \actionrv \sim \policy(\cdot \mid \staterv)}}  \left[ \grad[\action]\qfunc[ ][{\policy}](\staterv, \policy(\staterv)) \grad[\outer] \policy[\param](\actionrv \mid \staterv)\right] \\ 
    \grad[\inner] \cumulutil(\outer, \inner) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\initstates][\policy]\\ \actionrv \sim \policy(\cdot \mid \staterv)}}  \left[ \grad[\action]\qfunc[ ][{\policy}](\staterv, \policy(\staterv)) \grad[\inner] \policy[\inner](\actionrv \mid \staterv)\right]
\end{align}


\begin{lemma}[Policy Envelope theorem]
Consider the marginal function $\marginalfunc$ associated with the zero-sum stochastic Stackelberg game $\game$. 
\begin{align}
    \grad[\param] \cumulutil(\state, \param, \otherparam) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\state][\policy]\\ \actionrv \sim \policy[\param](\cdot \mid \staterv)}}  \left[ \qfunc[ ][{(\policy[\param], \policy[\otherparam])}](\staterv, \actionrv)  \grad[\param] \policy[\param](\actionrv \mid \staterv) \right]\label{eq:grad_x_cumulregret}\\
    \grad[\otherparam] \cumulutil(\state, \param, \otherparam) = \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\state][\policy]\\ \actionrv \sim \policy[\param](\cdot \mid \staterv)}}  \left[ \qfunc[ ][{(\policy[\param], \policy[\otherparam])}](\staterv, \actionrv)  \grad[\otherparam] \policy[\otherparam](\actionrv \mid \staterv) \right] \label{eq:grad_y_cumulregret} \\
    \grad[\policy] \exploit(\state, \param)  =  \mathop{\Ex^{\policy}}_{\substack{\staterv \sim \statedist[\state][\policy]\\ \actionrv \sim \policy[\param](\cdot \mid \staterv)}}  \left[ \qfunc[ ][{(\policy[\param], \policy[{\otherparam^*(\param)}])}](\staterv, \actionrv)  \grad[\param] \policy[\param](\actionrv \mid \staterv) \right]\label{eq:grad_x_exploit}
\end{align}
\end{lemma}
\begin{proof}
    \Crefrange{eq:grad_x_cumulregret}{eq:grad_y_cumulregret} follow directly from the policy gradient theorem \cite{sutton1999policy}, while \label{eq:grad_x_exploit} follows from \Cref{eq:grad_x_cumulregret} and the envelope theorem \cite{afriat1971envelope,milgrom2002envelope}.
\end{proof}
Note that the difference between \Cref{eq:grad_x_cumulregret} and \Cref{eq:grad_x_exploit} lies in the action-value function being computed w.r.t. to the best-response parameters $\otherparam^*(\param)$.

We first turn our attention to settings in which a minimax theorem holds such that:
% \begin{align}
$
\min_{\param \in \params} \max_{\otherparam \in \otherparams} \cumulutil(\state, \param, \otherparam) = \max_{\otherparam \in \otherparams} \min_{\param \in \params} \cumulutil(\state, \param, \otherparam)
$
% \end{align}
% 
allowing us to interpret the problem as a simultaneous-move game.



\deni{Add something on Noah Haipang's result}




\section{Regularized Exploitability}

\begin{restatable}[Parameteric Moreau Envelope Theorem]{theorem}{thmMoreauEnvelope}
\label{thm:moreau_envelope}
Given $\regulparam > 0$,
consider the parametric Moreau envelope $\exploit[\regulparam](\action) \doteq \max_{\otheraction \in \actions} \left\{\cumulutil (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2 \right\}$
and the associated proximal operator $\{\otheraction^*(\action)\} \doteq \argmax_{\otheraction \in \actions} \left\{\cumulutil (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2 \right\}$, %$\{\otheraction^*(\action)\} \doteq \argmax_{\otheraction \in \actions} \left\{\cumulutil (\action, \otheraction) - \frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2 \right\}$
where $\cumulutil$ is $\lipschitz[{\grad \cumulutil}]$-Lipschitz smooth.
%associated with the regularized cumulative regret function $\cumulutil[\regulparam]$:
% \begin{enumerate}
%     \item $\cumulutil[\regulparam]$ is $\regulparam$ strongly concave in $\otheraction$, and for all $\action \in \actionspace$, the set $\calB^*(\action)$ is a singleton.
%     \item For any SE $(\action^*, \otheraction^*)$ of $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$,  $\action^*= \otheraction^*$. Additionally, $\action^*$ is a SE strategy of the outer player iff $\action^*$ is a VE of $\pgame$.\amy{this is the point i am not getting up above, but which seems important, so let's try to improve the discussion above!}
%     \item 
Then $\exploit[\regulparam](\action)$ is $\left(\lipschitz[{\grad \cumulutil}] +  \frac{\lipschitz[{\grad \cumulutil}]^2}{\regulparam} \right)$-Lipschitz-smooth, with gradients $\grad[{\action}] \exploit[\regulparam](\action) = \grad[{\action}] \cumulutil(\action, \otheraction^*(\action)) -  \regulparam(\action[][] - \otheraction[][]^*(\action))$.
% \end{enumerate}
\end{restatable}


\begin{restatable}{theorem}{lemmaLipschitzSmoothVal}
\label{lemma:lipschitz_smooth_val}
Given $\regulparam > 0$,
the following properties hold for $\regulparam$-regularized exploitability %$\exploit[\regulparam](\action) \doteq \max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$
and its associated solution correspondence $\calB^*(\action) \doteq \argmax_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$:
%associated with the regularized cumulative regret function $\cumulutil[\regulparam]$:
\begin{enumerate}
    \item $\cumulutil[\regulparam]$ is $\regulparam$ strongly concave in $\otheraction$, and for all $\action \in \actionspace$, the set $\calB^*(\action)$ is a singleton.
    
    \item For any SE $(\action^*, \otheraction^*)$ of $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$,  $\action^*= \otheraction^*$. Additionally, $\action^*$ is a SE strategy of the outer player iff $\action^*$ is a VE of $\pgame$.
    % \amy{this is the point i am not getting up above, but which seems important, so let's try to improve the discussion above!}
    
    \item $\exploit[\regulparam](\action)$ is $\left(\lipschitz[{\grad \cumulutil[\regulparam]}] +  \frac{\lipschitz[{\grad \cumulutil[\regulparam]}]^2}{\regulparam} \right)$-Lipschitz-smooth with gradients given by for all $\player \in \players$:
    $$\grad[{\action[\player]}] \exploit[\regulparam](\action) =  \sum_{\player \in \players}  \left[ \grad[{\action[\player]}] \util[\player](\otheraction[\player][]^*(\action), \naction[\player][]) - \grad[{\action[\player]}] \util[\player](\action[\player][][], \naction[\player][]) \right]  -  \regulparam(\action[\player][] - \otheraction[\player][]^*(\action)) $$
    \noindent where $\{\otheraction^*(\action)\} = \calB^*(\action)$
\end{enumerate}
\end{restatable}


\begin{proof}


\noindent
(1) Notice that $\cumulutil(\action, \otheraction)$ is concave in $\otheraction$ for all $\action \in \actionspace$, hence, since $\frac{\regulparam}{2} \left\| \action - \otheraction \right\|_2^2$ is $\regulparam$-strongly convex in $\otheraction$, $ \cumulutil[\regulparam](\action, \otheraction)$ is strongly concave in $\otheraction$, and $\argmax_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$ must be singleton-valued.


\noindent
(2) First, note that a Stackelberg equilibrium of $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$ is guaranteed to exist by continuity of $\cumulutil[\regulparam]$ and compactness of the constraints. 

\noindent 
(SE $\Leftarrow$ VE): 
Suppose that $\action^* \in \actions$ is a VE of $\pgame$, then for all $\otheraction \in \actionspace$ we have:
\begin{align}
    \cumulutil[\regulparam](\action^*, \otheraction) 
    &= \cumulutil(\action^*, \otheraction) - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2\\
    &= \sum_{\player \in \players} \left[ \underbrace{\util[\player](\otheraction[\player], \naction[\player]) - \util[\player](\action[\player], \naction[\player])}_{\leq 0 \text{ by GNE definition}} \right] - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2 \\
    &\leq - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2
\end{align}

Taking the max over $\otheraction$ on both sides of the final inequality, we obtain $$\max_{\otheraction \in \actions} \cumulutil[\regulparam](\action^*, \otheraction) \leq \max_{\otheraction \in \actions} - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2 \leq 0 \enspace .$$ 
Note that for all $\action \in \actions$, $\max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction) 
\geq \cumulutil[\regulparam](\action, \action) = 0$, hence we must have that $\action^*$ is the SE strategy of the outer player and the SE strategy of the inner player $\otheraction^*$ must be equal to $\action^*$.


(SE $\Rightarrow$ VE): \deni{NEEDS TO GET FIXED} Let $(\action^*, \otheraction^*)$ be an SE of $\min_{\action \in \actions} \max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction)$. Note that for all $\action \in \actions$, $\max_{\otheraction \in \actions} \cumulutil[\regulparam](\action, \otheraction) \geq \cumulutil[\regulparam](\action, \action) = 0$.
Since under our assumptions a GNE is guaranteed to exist, there exists $\action^\prime$ such that $\max_{\otheraction \in\actionspace} \cumulutil[\regulparam](\action^\prime, \otheraction) = 0$, we must then have that $\min_{\action \in \actions} \max_{\otheraction \in\actionspace} \cumulutil[\regulparam](\action, \otheraction) \leq 0$, i.e.:
\begin{align}
    \max_{\otheraction \in\actions} \left\{ \sum_{\player \in \players} \left[ \util[\player](\otheraction[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2 \right\} \leq 0
\end{align}


We will show that the exploitability of $\action^*$ is zero w.r.t. the pseudo-game $\pgame$, which will imply that $\action^*$ is a GNE. First, by the above equation, we have for any $\otheraction \in \actionspace$:

\begin{align}
\sum_{\player \in \players} \left[ \util[\player](\otheraction[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2 \leq 0    
\end{align}

For $\lambda \in (0,1)$, and any $\action \in \actionspace$,  let $\otheraction[\player] = \lambda \action[\player]^* + (1 - \lambda) \action[\player]$ in the above inequality, we then have:

\begin{align}
0 &\geq \sum_{\player \in \players} \left[ \util[\player](\lambda \action[\player]^* + (1 - \lambda) \action[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} \left\| \action^* - [ \lambda \action^* + (1 - \lambda) \action ]\right\|_2^2   \\
&= \sum_{\player \in \players} \left[ \util[\player](\lambda \action[\player]^* + (1 - \lambda) \action[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} \left\| (1- \lambda) \action^*  - (1 - \lambda) \action \right\|_2^2  \\
&= \sum_{\player \in \players} \left[ \util[\player](\lambda \action[\player]^* + (1 - \lambda) \action[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} (1- \lambda)^2 \left\| \action^* - \action\right\|_2^2 \\
&\geq \sum_{\player \in \players} \left[ \lambda \util[\player]( \action[\player]^*, \naction[\player][][][*]) +  (1 - \lambda) \util[\player](\action[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} (1- \lambda)^2 \left\| \action^* - \action[\player ]\right\|_2^2 \\
\end{align}
Taking $\lambda \to 1^-$, by continuity of the $l_2$-norm and the utility functions, we have:
\begin{align}
    0 \geq \sum_{\player \in \players} \left[ \util[\player]( \action[\player]^*, \naction[\player][][][*])  - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right]
\end{align}
which implies that $\action^*$ is a GNE, additionally for $\sum_{\player \in \players} \left[ \util[\player](\otheraction[\player], \naction[\player][][][*]) - \util[\player](\action[\player]^*, \naction[\player][][][*]) \right] - \frac{\regulparam}{2} \left\| \action^* - \otheraction \right\|_2^2 \leq 0$ to be minimized by $\action^*$, we must have that $\otheraction = \action^*$.

(3): Follows from \Cref{thm:moreau_envelope}.

\end{proof}


\begin{lemma}[Inner Loop Error Bound]

\end{lemma}

\begin{lemma}[Lipschitz smooth exploitability]
    
\end{lemma}


\begin{lemma}[Outer loop progress bound]
    
\end{lemma}

\begin{theorem}[Convergence Result]
    
\end{theorem}

\begin{algorithm}[!h]
\caption{Augmented Descent Ascent (ADA)}
\textbf{Inputs:} $\numplayers, \util, \regulparam, \learnrate[\action], \learnrate[\otheraction], \numiters[\action], \numiters[\otheraction], \action[][][0], \otheraction[][][0]$\\
\textbf{Outputs:} $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^{\numiters[\action] }$
\label{alg:cumul_regret}
\begin{algorithmic}[1]
\For{$\iter = 0, \hdots, \numiters[\action] - 1$}
    % \For{$\player \in \players$}
    \State
    $\action[][][\iter+1] = \project[\actions] \left[\action[][][\iter] - \learnrate[\action] \left(  \grad[{\action[]}] \cumulutil(\action[][][\iter], \otheraction[][][\iter])   -  \regulparam(\action[][][\iter] - \otheraction[][][\iter]) \right) \right]$
    % \EndFor
    
    \State $\otheraction[][] = \zeros$
    
    \For{$s = 0, \hdots, \numiters[\otheraction] - 1$}
        % \For{$\player \in \players$}
        \State $\otheraction[][]  = \project[\actions] \left[ \otheraction[][][] + \learnrate[\otheraction] \left(\grad[{\otheraction}]\cumulutil(\action[][][\iter + 1], \otheraction) - \regulparam(\action[][][\iter + 1] - \otheraction[][]) \right) \right]$
    % \EndFor
    \EndFor
    
    \State $\otheraction[][][\iter + 1] =  \otheraction$
    
    \EndFor
\State \Return $(\action[][][\iter], \otheraction[][][\iter])_{t = 0}^{\numiters[\action]}$
\end{algorithmic}
\end{algorithm}

